An Algorithmic Framework for Efficient Large-Scale Circuit Simulation Using Exponential Integrators

We propose an efficient algorithmic framework for time domain circuit simulation using exponential integrator. This work addresses several critical issues exposed by previous matrix exponential based circuit simulation research, and makes it capable of simulating stiff nonlinear circuit system at a large scale. In this framework, the system's nonlinearity is treated with exponential Rosenbrock-Euler formulation. The matrix exponential and vector product is computed using invert Krylov subspace method. Our proposed method has several distinguished advantages over conventional formulations (e.g., the well-known backward Euler with Newton-Raphson method). The matrix factorization is performed only for the conductance/resistance matrix G, without being performed for the combinations of the capacitance/inductance matrix C and matrix G, which are used in traditional implicit formulations. Furthermore, due to the explicit nature of our formulation, we do not need to repeat LU decompositions when adjusting the length of time steps for error controls. Our algorithm is better suited to solving tightly coupled post-layout circuits in the pursuit for full-chip simulation. Our experimental results validate the advantages of our framework.

==> abstract.tex <==

This paper proposes an efficient time-domain integration method for simulating power distribution networks, including nonlinear devices. The algorithm is based on matrix exponential method and  

Time-domain circuit simulation using exponential method 
has many advantages, such as large time stepping,  stability. Previous,  matrix exponential-based methods \cite{Weng12_TCAD} \cite{Weng12_ICCAD} suffer the memory and runtime constraints from stiff circuit system. Those methods also require regularization to keep the storage element matrix non-singular. Above factors limit the scope of application. On the other hand, in current industry and academic, robust and standard method to solve general nonlinear circuit simulation is Newton-Raphson backward Euler method. However, it sometimes requires many iterations of solving linear system (e.g. LU solving) in order to satisfy the convergence condition as well as the truncation error budget. All degrade the performance of simulator.

In this work, we equip matrix exponential-based numerical integration kernel with exponential Rosenbrock-Euler method and Krylov subspace using inverted matrix bases. We remove the regularization process, reduce LU operations for each time stepping. We pose LU only on conductance/resistance matrix, which is much sparser than capacitance/inductance matrix after extraction. This property cannot be achieved non-matrix exponential-based integration kernels, due to the requirement of differential equation approximation. Therefore, such method can be much more robust for simulating strong parasitic cases. 
The experimental results show large speedups.




==> adaptive_step_control.tex <==
The proposed MEXP can significantly benefit from the adaptive time stepping because the rational Krylov subspace approximation 
relaxes the stiffness constraint as well as preserves the scaling invariant property. As a result, MEXP can effortlessly adjust 
the step size to different scale,
%e.g., from 1\emph{ps} to 1\emph{ns}, 
during the simulation. Such adaptivity is particularly 
helpful in the power grid where the voltage noise includes the high- to low-frequency responses from die, package and board. 

Our adaptive step scheme is to step forward as much as possible so that MEXP can quickly finish the simulation.  With the 
insight from Eqn. (\ref{eq:scale}), MEXP can adjust $\alpha$ to calculate results of required step sizes with only one 
Arnoldi process. However, even though the rational Krylov subspace could scale 
%arbitrarily
robustly, the step size in MEXP is restrained 
from input sources. As shown in Eqn.~(\ref{eqn:pwl_exact_sol}), MEXP has to guarantee constant slope during a stepping, and hence 
the maximum allowed step size $h$ at every time instant is limited. Our scheme will first determine $h$ from inputs at 
time $t$ and construct the rational Krylov subspace from $\mbf{x}(t)$. Then, $\mbf{x}$ within interval $[t,~t+h]$ are 
calculated through the step size scaling. 

Algorithm~\ref{algo:adaptive_step} shows MEXP with adaptive step control. In order to comply with the required accuracy during the 
simulation, the allowed error $err(m,\alpha)$
at certain time instant $t$ is defined
as $ err \le \frac{E_{Tol}}{T}h $
where $E_{Tol}$ is the error tolerance in the whole simulation process, $T$ is the simulation time span, $h$ is the 
step size at time $t$, and $err$ is the posterior error of MEXP from Eqn. (\ref{eq:post_err_est}). Hence, when 
we construct the rational Krylov subspace, we will increase $m$ until the $err(m,\alpha)$ satisfies the error tolerance. 
%\vspace{-0.1in}
\begin{algorithm} 
    \label{algo:adaptive_step}
    \caption{Hybrid MEXP with Adaptive Step Control}
    \KwIn{$\mbf{C}$, $\mbf{G}$, $\mbf{B}$, $\mbf{u}(t)$, $\tau$, $\gamma$, error tolerance $E_{Tol}$ and simulation time $T$ with predefine constant  $ m_{min}, c_{onst} $}
    \KwOut{$\mbf{x}(t)$}
    {
        $t = 0$\; 
         $\mbf{x}(0)$ = DC\_analysis\;
        %Choose $\tau$ for rational Krylov subspace method\;
        $[\mbf{L}_{sub},\mbf{U}_{sub}] = $LU($\mbf{C} +\gamma \mbf{G}$)\;
        \While{$t \leq T$}
        {	
	    %Update $v_{k+1}$ with $\mbf{L}, \mbf{U}, \mbf{W}$ by (\ref{eq:blu_f})\;
	    %and update $\mathbf{L},\mathbf{U}$ by (\ref{eq:blu})\;
%	    At time point $t_k$, 
   		\tcp{Try jump as furthest as possible.}
	    Compute maximum  allowed step size $h$ from $\mbf{u}(t)$ and
	    $\alpha = \frac{h}{\gamma}$ \; 	   
	    
   	    \If {$\alpha \in [1, m_{min}+c_{onst}]$   	    } 
	    {
	        \tcp{Marching with medium time step uses TRAP
	        Why "medium"? The time step resolution is not limited by LTE, it is limited
	        by the smallest transition period of input, e.g. $10^{-11}s$ among $10^{-8}$
	        time span simulation. 
	        }
	        $t_{anchor} = t$\; 
	    	\While {$t < t_{anchor} + h$ }
	    	{
	    		Use $\mbf L_{sub}$ and $\mbf U_{sub}$ directly for TRAP\; 
	    		$t = t+ \gamma * 2 $\;\tcp{Use TRAP }
	    	}
	    }
	    \Else{
	    
	    \tcp{Large step size striding.}
	    Construct $\mbf{H_{m,m}}$, $\mbf{V_{m,m}}$, $err$ by Arnoldi process 
	    and (\ref{eq:post_err_est}) 
	    until $err(m,\alpha) \le \frac{E_{Tol}}{T}h$\;
	    Compute $\mbf{x}(t+h)$ by (\ref{eq:scale})\;
	    	    $t = t+h$;
	    }
 	    }
	}
\end{algorithm}
%\vspace{-0.1in}
The complexity of MEXP with adaptive time stepping is mainly determined by the total number of required backward/forward
substitutions
during the simulation process. 
%This is because the dimension of $\mbf{H_m}$ is small,
%, e.g., around $4 \sim 20$, 
%and then computation overhead of the step size scaling is negligible.
The number of total substitution 
operations is 
$    \sum_{i=0}^N m_{i} $
where $N$ is total time steps, and $m_i$ is required dimension of the rational 
Krylov subspace at time step $i$. Compared 
to the trapezoidal method where the number of substitution operations depends only on the fixed step size,
 MEXP could use less 
substitution operations as long as the maximum allowed
step size $h$ is much larger than the fixed step size. Our 
experiments in the following section demonstrates it is usually the case for the power grid simulation.





==> dac14_nl_er.tex <==
%{\color{red} clear $D_j$ notation and add motivation, point out the important advantages! }
%\subsection{Motivation} 
%The {\bf motivation} ... 
Our  circuit solver is based on
%matrix exponential time-integration kernel with 
exponential Rosenbrock-type formulation and still use matrix exponential as time integration kernel.  
We discuss classic exponential Rosenbrock-Euler and, then Rosenbrock-type methods with multiple stages. We also demonstrate how the mathematical formulations are applied to SPICE-like simulation. 
\subsection{Circuit Solver using Exponential Rosenbrock-Euler Framework}
First, we discuss the general mathematical formulation for dynamical system. Then, we apply this formulation for SPICE-like formulation. 
\subsubsection{Formulation for Dynamical System}
%\begin{eqnarray}
%\mbf F_n(\mbf x_n) = \frac{\partial f}{\partial  t} (\mbf x, \mbf u, t_n) 
%\end{eqnarray} 
%$\mbf J_n$ is the Jacobian of $\mbf F$, and $\mbf g_n$ is the nonlinear remainder, which are evaluated at $\mbf x_n$.
To derive such method for SPICE-like circuit solver, we first consider non-autonomous system
%\begin{eqnarray}
$\frac{d\mvect x(t)}{dt} = \mvect  g(\mvect x, \mvect u,t)$. 
We have so-call exponential (one-stage) 
Rosenbrock-Euler  formulation \cite{Hochbruck09_RB, Caliari09_ER, Carr13}:
\begin{eqnarray}
\mvect x_{k+1} =  \mvect  x_{k} + h_k \phi_1(h_k \mbf J_k) \mvect g(\mbf x_k,\mvect u, t_k)+h^2_k\phi_2(h_k\mbf J_k)\mvect b_k
\label{eq_rbeuler}
\end{eqnarray}
where 
%\begin{eqnarray}
%\mbf J_n = \frac{\partial f}{\partial \mbf x} (\mbf x, \mbf u, t_n), ~~
$\mbf J_k  $ denotes the Fr\'{e}chet derivative of $\mvect g$,
%\begin{eqnarray}
$
\mvect b_k = \frac{\partial  \mvect g}{\partial  t} (\mvect x_k, \mvect u, t_k) 
$,
%\end{eqnarray}  
then $\mbf b_k = \mvect 0$ for autonomous system.
Function $\phi_{i}(z)$ is defined as  
%\begin{eqnarray}
$\phi_{i}(z) =  \int_{0}^1 e^z(1-s)\frac{s^{i-1}}{(i-1)!}ds  ~~(i \ge 1),  
$
%\end{eqnarray}
which leads to 
\begin{eqnarray}
\phi_{i+1}(h_k \mbf J_k) =  \frac{\phi_i(h_k \mbf J_k) - \phi_i(\mathbf 0)}{h_k \mbf J_k}  , ~~ \phi_{0}(h_k \mbf J_k) = \mbf e^{h_k \mbf J_k}
\end{eqnarray}
%and $\phi_{0}(h_k \mbf J_k) = \mbf I $. 
For example, 
%\begin{eqnarray}
$\phi_1(h_k \mbf J_k) = \frac{e^{h_k \mbf J_k } - \mbf I_n}{h_k \mbf J_k} , ~~~
\phi_2(h_k \mbf J_k) = \frac{ \phi_1(h_k \mbf J_k) - \mbf I_n}{h_k \mbf J_k}$.
% \end{eqnarray} 
% \nonumber
%\phi_3(h_n \mbf J_n) &=& \frac{ \phi_2(h_n \mbf J_n) - \frac{1}{2}\mbf I}{h_n J_n}
%\end{eqnarray}
The advantage of Eq. (\ref{eq_rbeuler}) is that is stable in the entire complex plane, which is superior to all of the backward differential formula methods \cite{Carr13}.
Therefore, those $\phi_i$ functions permit a large value for the step size $h_k$. 
%where $\mbf J_n = \mbf g( \mbf x_n, \mbf u, t_n)$, and
%It is a second order exponential Rosenbrock-type method.

%$\mbf J_n = \frac{\partial \mbf F}{\partial \mbf x} (\mbf x_n, t_n), ~\mbf g_n (\mbf x_n) = \mbf F(\mbf x_n, t_n)-\mbf J_n \mbf x_n$
%\subsection{Exponential Rosenbrock-Euler Formulation of MNA-based Circuit Simulation}
\vspace{+0.08in}
\subsubsection{Formulation for Circuit Solver}
To apply exponential Rosenbrock-Euler method to SPICE-like circuit simulation formulation Eq. (\ref{eq_mna}), 
%the formulation is shown as follows,
%is relative dense compared to non-post-layout version, leading to 
%\begin{eqnarray}
%(\mbf C_l + \mbf C_{nl} ) \frac{d \mbf x(t)}{dt} + (\mbf G_l + \mbf G_{nl} ) \mbf x(t)  = \mbf B \mbf u(t)  + \mbf I_{cur}
%\end{eqnarray}
%\begin{eqnarray}
%\mbf C (\mbf x(t)) \frac{d \mbf x(t)}{dt} + \mbf G \mbf x(t)  = \mbf B \mbf u(t)  + \mbf I_{cur}
%\end{eqnarray}
%first, we assume $\mbf C(\mbf x(t))$ is invertible (the assumption is nt  necessary, 
%because the directly factorization of $\mbf C(\mbf x(t))$ is avoided within Krylov subspace approximation in Sec. \ref{sec:exp_krylov} or \cite{Zhuang14_DAC}). 
We start from Eq. (\ref{eq_mna}) 
%\begin{eqnarray}
%\frac{d \mbf x(t)}{dt} + \mbf C(\mbf x(t))^{-1} \mbf G \mbf x(t)   = \mbf C(\mbf x(t))^{-1} \mbf B \mbf u(t)   + \mbf C(\mbf x(t))^{-1} \mvect F(\mbf x(t))
%\end{eqnarray}
to model corresponding non-autonomous dynamical system is 
\begin{eqnarray}
\frac{d\mvect x(t)}{dt}  = 
\mvect  g(\mvect x, \mvect u,t)=  -\mbf J_k  \mvect x(t) 
%\nonumber \\
  + \mbf C^{-1}\left(\mvect x(t)\right)  \mvect F \left (\mvect x(t) \right)  \nonumber \\ +  \mbf C^{-1}\left(\mvect x(t)\right)  \mbf B \mvect u(t)  
\end{eqnarray}
%More generally,
where $\mbf J_k = -\mbf C^{-1} (\mvect x_k)  \mbf G(\mvect  x_k)$. The nonlinear remainder $\mvect d_k(\mvect x ) = \mvect g(\mvect x_k , \mvect u, t_k) - \mbf J_k \mvect x -  t_k \mvect b_k $ with 
$\mvect b_k =   \mbf C^{-1}(\mvect x_k)  \mbf B \frac{\partial \mvect u (t) }{\partial t} $
  \begin{eqnarray}
  \phi_{i+1}(h_k \mbf J_k) =  \frac{1}{h_k} \left( \phi_i(h_k \mbf J_k) -\mbf I \right) \mbf T_k
  \end{eqnarray}
  where $\mbf T_k = -\mbf G^{-1}(\mvect x_k) \mbf C (\mvect x_k) $. 
\begin{comment}
  Therefore,
\begin{eqnarray}
\phi_1(h_k \mbf J_k) &=& - \frac{1}{h_k} \left( e^{h_k \mbf J_k} -\mbf I   \right) \mbf G^{-1}(\mvect x_k) \mbf C (\mvect x_k) \\
\phi_2(h_k \mbf J_k) &=& - \frac{1}{h_k} \left( \phi_1(h_k \mbf J_k) -\mbf I \right) \mbf G^{-1}(\mvect x_k) \mbf C (\mvect x_k) %\nonumber
 \\
& = &  \frac{1}{h_k^2} \left( e^{h_k \mbf J_k} -\mbf I   \right) 
%\mbf G^{-1}(\mvect x_k) \mbf C (\mvect x_k)\mbf 
\left( G^{-1}(\mvect x_k) \mbf C (\mvect x_k) \right)^2 + \frac{1}{h_k}  \mbf G^{-1}(\mvect x_k) \mbf C (\mvect x_k)  \nonumber  
%\phi_3(h_n \mbf J_n) &=& - \frac{1}{h_n} (\phi_2(h_n \mbf J_n) -\frac{1}{2}\mbf I)\mbf G^{-1} \mbf C 
\end{eqnarray}
\end{comment}
%$\mvect b_k = \mbf G(\mvect x_k)^{-1} \mbf C(\mvect x_k)\mbf G(\mvect x_k)^{-1}  \mbf B  \frac{ \mvect u( h_{k+1}) - \mvect u(t_k)}{h_k}$  
Therefore, solution by Eq. (\ref{eq_rbeuler})
\begin{eqnarray}
\Theta_{1}(h, \mvect x_{k,0}) = \frac{1}{h }  \left(e^{h  \mbf J_k} -\mbf I_n \right) \mbf T_k \mvect x_{k,0}   
\end{eqnarray} 
where 
$ \mvect x_{k,0}  = -\mbf C^{-1}(\mvect x_k) \mbf G  (\mvect x_k)\mvect x_k + \mbf C^{-1}(\mvect x_k)  \left(  \mvect F(\mvect x_n) +  \mbf B \mvect u(t_n) \right)$. 
 % $\mvect x_{k,1}  =  -\mbf G^{-1}(\mvect x_k) \mbf C^{-1} (\mvect x_k) \mvect x_{k,0}$
%\begin{eqnarray} &&
 %  \mvect x_{k,1}  = \mvect x_k -  \mbf G^{-1}(\mvect x_k)  \left(  \mvect F(\mvect x_n) +  \mbf B \mvect u(t_n) \right)$
%  \label{eq_two_vec1} 
%\end{eqnarray}
\begin{eqnarray} 
\Theta_{2}(h, \mvect b_{k,0}) = \frac{1}{h } \mbf T_k \mvect b_{k,0} +   \frac{1}{h ^2}  \left( e^{h \mbf J_k} -\mbf I_n \right) \mbf T^2_k \mvect b_{k,0}   %\nonumber  %\\
   % &+ & h_n  \mbf G(\mbf x_n)^{-1} \mbf C(\mbf x_n) \mbf G(\mbf x_n)^{-1} \mbf B  \frac{ \mbf u(t+h_n) - \mbf u(t_n)}{h_n}
\end{eqnarray}
%\begin{eqnarray}
 Assume $\mvect u(t)$ is a piecewise-linear function when $t \in (t_k,t_{k+1}]$, $\mvect b_{k,0} =   \mbf C^{-1}(\mvect x_k) \mbf B  \frac{ \mvect u(t_{k+1}) - \mvect u(t_k)}{h_k}
    \label{eq_two_vec1}$.  %$\mvect b_{k,1} =  \mbf G^{-1}(\mvect x_k) \mbf C(\mvect x_k)  \mvect b_{k,0} =   \mbf G^{-1}(\mvect x_k) \mbf B  \frac{ \mvect u(t_{k+1}) - \mvect u(t_k)}{h_k}     \label{eq_two_vec2}$, 
  % and $\mvect b_{k,2}=  -\mbf G^{-1}(\mvect x_k) \mbf C(\mvect x_k)         \mvect b_{k,1}        $.
       %\mbf G^{-1}(\mvect x_k) \mbf B  \frac{ \mvect u(t_{k+1}) - \mvect u(t_k)}{h_k}
      %\label{eq_two_vec2} 
%\end{eqnarray}

The solution by exponential Rosenbrock-Euler method is 
%\begin{eqnarray}
 \begin{empheq}[box=\fbox]{align}
 \mvect x^{(1)}_{k+1}(h_k) = \mvect x_k + h_k \Theta_1 (h_k, \mvect x_{k,0}) + h_k^2 \Theta_{2}  (h_k, \mvect b_{k,0} %\mvect v_{22}
 )
   \label{eq_rbe}
 \end{empheq}
%\end{eqnarray} 
%  Furthermore, 
\begin{comment}
 \begin{eqnarray}
 \mvect x_{k+1} = \mvect x_k  +  e^{h_k \mbf J_k}\mvect v_1 - \mvect v_1  + e^{h_k \mbf J_k}
 %\mbf G^{-1}(\mvect x_k) \mbf C(\mvect x_k) 
 \mvect v_2 
 - \mvect v_2
 %\nonumber \\
 %&+& \mbf G^{-1} \mbf C \mbf G^{-1} \mbf B  ( \mbf u(t+h_n) - \mbf u(t) ) \nonumber \\
 +  h_k \mvect v_3  
 \label{eq_solver}
 \end{eqnarray}
\end{comment}
%where $\mvect X^{(i)}_{s}$ denotes the operation in $s$-stage method for $\phi_i$ function and vector product
%{\color{red} We parameterize the $\mvect X_1^{(1)}(h)$, $\mvect X_2^{(1)}(h)$, etc, in order to make programming and reuse intermediate results more easily.}
%There are two MEVPs $e^{h_n \mbf J_n} \mvect v_1$ 
%and $e^{h_n\mbf J_n} \mvect v_{22} $,  
%$e^{h_n\mbf J_n}  \left( \mbf G^{-1}(\mvect x_k) \mbf C(\mvect x_k)\mbf v_2\right)$, 
%to be evaluated, which we apply a fast method to compute MEVPs via Krylov subspace in Sec. \ref{sec_krylov}. 
The error estimator is a crucial ingredient of controlling time step. Caliari and Ostermann \cite{Caliari09_ER} devised a formula to estimate local nonlinear truncation error as
\begin{eqnarray}
  \label{eqn_expRB2_err}
    e^{(1)}_{rr} (\mvect x_{k+1},\mvect x_k) %\mbf {x_{n+1}} - \mbf x_{n+1}  \\
   =
  h_k \phi_1 (h_k \mbf J_k) ( \mvect d_k(\mvect x_{k+1},\mvect u, t_{k+1}) - \mvect d_k( \mvect x_k,\mvect u, t_k) )  \\
  = - ( e^{h_k \mbf J_n} -\mbf I )\mbf T_k ( \mvect d_k(\mvect x_{k+1},\mvect u, t_{k+1}) - \mvect d_k( \mvect x_k,\mvect u, t_k) )  
  %&=&  -\mbf V_m (e^{h_n \mbf H_n} -\mbf I) \mbf G^{-1}  ( \mbf I_{cur}(\mbf x_{n+1}) - \mbf I_{cur}(\mbf x_n ) )  
  \nonumber
\end{eqnarray} 
 

%\vspace{+0.08in}
\subsection{Circuit Solver using Multi-Stage Exponential Rosenbrock-Type Methods} 
%\subsection{Multiple-Stage Exponential Rosenbrock-Type Extensions} 
\subsubsection{Formulation of Dynamical System}
The solution has a generalized form $s$-stage exponential Rosenbrock-Type methods %, which can be viewed as extra term to increase the accuracy order of exponential Rosenbrock-Euler methods 
\cite{Hochbruck09_RB, Caliari09_ER}.
\begin{eqnarray}
\mvect X^{(s)}_{ki} &=& \mvect x_k+ c_i h_k \phi_1(c_i h_k \mbf J_k)\mvect g(\mvect x_k,\mvect u, t_k) +  c_i^2 h_k^2 \phi_2(c_i h_k \mbf J_k)\mvect b_k  \nonumber \\
& +& h_k \Sigma_{j=2}^{i-1}a_{ij}(h_k \mbf J_k) \mvect D_{k}(\mvect X_{kj}) %(\mvect X_{ki})  
\\
\mvect x^{(s)}_{k+1} &=& \mvect x_k+  h_k \phi_1( h_k \mbf J_k)\mvect g(\mvect  x_k,\mvect u, t_k) + h_k^2 \phi_2( h_k \mbf J_k)\mvect b_k  \nonumber \\ &+& h_k \Sigma_{i=2}^{s}b_{i}(h_k \mbf J_k) \mvect D_{k} (\mvect X_{ki})%(\mvect X_{ki})
%\nonumber
\label{eq_rb_series}
\end{eqnarray}
where 
$\Sigma_{i=1}^s b_i(z) = \phi_1(z) $, 
$\Sigma_{j=1}^{i-1} a_{ij}(z) = c_i\phi_1(c_iz), ~~ ~ 1\le i \le s$, $c_1=0$, 
%\mvect d_k( \mvect x, \mvect u, t) &=& \mvect g(\mvect x , \mvect u, t) - \mbf J_k \mvect x - \mvect b_k t \\ 
%
\begin{eqnarray}
\mvect D_{k}(\mvect X_{j}) = \mvect d_k( \mvect X_{j}, \mvect u, t_k+c_jh_k)- \mvect d_k( \mvect x_k, \mvect u,  t_k)
\end{eqnarray}
\begin{comment}
\begin{eqnarray}
\mvect X_{ki} = e^{c_ih_k\mbf J_k} \mvect x_k + h_k \Sigma_{j=1}^{i-1} a_{ij}(h_k \mbf J_k) \mvect g_i(\mvect X_{kj})   \\
\mvect x_{k+1} = e^{ h_k\mbf J_k} \mvect x_k + h_k \Sigma_{i=1}^{s} b_i(h_k \mbf J_k) \mvect g_i(\mvect X_{kj})
 % \label{eq_rb_series}
\end{eqnarray}
\end{comment}
Eq.(\ref{eq_rb_series}) is the final solution for next time step $\mvect x_{k+1}$. 
%When we remove the term $h_k\Sigma_{i=2}^{s}b_{i}(h_k \mbf J_k)D_{ki}(\mvect X_{ki})$ from 
%Eq. (\ref{eq_rb_series}) is back to exponential Rosenbrock-Euler formulation.
$\mvect D_{k}(\mvect X_{ki})$ are expected to be small in norm and can be cheaply computed. 
There are several common adopted strategies, e.g. 2-stage, and 3-stage  exponential Rosenbrock-Type methods \cite{Hochbruck09_RB}: 
\begin{comment}
\begin{eqnarray}
\mvect X_{k1} = \mvect x_k+ c_i h_k \phi_1(c_ih_k \mbf J_k)\mvect g(\mvect x_k) +  c_i^2 h_k^2 \phi_2(c_ih_k \mbf J_k)\mvect b_k   \\ + h_k \Sigma_{j=2}^{i-1}a_{ij}(h_k \mbf J_k) \mvect D_{kj} \nonumber\\
\mvect X_{k2} = \mvect x_k+ c_i h_k \phi_1(c_ih_k \mbf J_k)\mvect g(\mvect x_k) +  c_i^2 h_k^2 \phi_2(c_ih_k \mbf J_k)\mvect b_k   \\ + h_k \Sigma_{j=2}^{i-1}a_{ij}(h_k \mbf J_k) \mvect D_{kj} \nonumber\\
\mvect x_{k+1} = \mvect x_k+  h_k \phi_1( h_k \mbf J_k)\mvect g(\mvect x_k) + h_k^2 \phi_2( h_k \mbf J_k)\mvect b_k   \\ + h_k \Sigma_{i=2}^{s}b_{i}(h_k \mbf J_k) \mvect D_{ki}\nonumber
 % \label{eq_rb_series}
\end{eqnarray}
\end{comment}


\vspace{+0.08in}
\subsubsection{Two-stage exponential Rosenbrock-Type Formulation} 

Hochbruck, Ostermann, and Schweitzer \cite{Hochbruck09_RB} proposed the two-stage exponential Rosenbrock-Type method as follows, 
\begin{eqnarray}
\mvect X^{(2)}_{k1} &=& \mvect x_k+  h_k \phi_1( h_k \mbf J_k)\mvect g( \mvect x_k,\mvect u, t_k) + h_k^2 \phi_2( h_k \mbf J_k)\mvect b_k 
\label{eq_2stage_1}
\nonumber\\ 
\mvect x^{(2)}_{k+1} &=& \mvect x_k+  h_k \phi_1( h_k \mbf J_k)\mvect g( \mvect x_k,\mvect u, t_k) + h_k^2 \phi_2( h_k \mbf J_k)\mvect b_k  \nonumber \\ 
&+&   2h_k\phi_3(h_k\mbf J_k)  \mvect D_{k}(\mvect X^{(2)}_{k1}) 
\label{eq_2stage_2}
\nonumber 
 % \label{eq_rb_series}
\end{eqnarray}
The error estimator \cite{Caliari09_ER, Hochbruck09_RB} is 
\begin{eqnarray}
e^{(2)}_{rr} = \mvect x_{k+1} - \mvect X^{(2)}_{k1} = 2h_k\phi_3(h_k\mbf J_k)  \mvect D_{k}(\mvect X^{(2)}_{k1}) 
\end{eqnarray}
%Eq. (\ref{eq_2stage_1}) is actually exactly same as Eq. (\ref{eq_rbe}).
\begin{comment}
where 
\begin{eqnarray}
 \phi_3(h_k \mbf J_k) & = &  - \frac{1}{h_k} \left( \phi_2(h_k \mbf J_k) -\mbf I \right) \mbf G^{-1}(\mvect x_k) \mbf C (\mvect x_k)  \\
 & = &  -\frac{1}{h_k^3} \left( e^{h_k \mbf J_k} -\mbf I   \right) 
 %\mbf G^{-1}(\mvect x_k) \mbf C (\mvect x_k)\mbf 
 \left( G^{-1}(\mvect x_k) \mbf C (\mvect x_k) \right)^3 
\nonumber   \\
& -& \frac{1}{h_k^2}   \left( G^{-1}(\mvect x_k) \mbf C (\mvect x_k) \right)^2 +
    \frac{1}{h_k}    G^{-1}(\mvect x_k) \mbf C (\mvect x_k)  \nonumber  
 %\phi_3(h_n \mbf J_n) &=& - \frac{1}{h_n} (\phi_2(h_n \mbf J_n) -\frac{1}{2}\mbf I)\mbf G^{-1} \mbf C 
%\phi_3(h_n \mbf J_n) &=& - \frac{1}{h_n} (\phi_2(h_n \mbf J_n) -\frac{1}{2}\mbf I)\mbf G^{-1} \mbf C 
\end{eqnarray}
\end{comment}
%The corresponding SPICE-like formulation, 
Then Eq. (\ref{eq_2stage_2}) is formed by adding  Eq. (\ref{eq_rbe}) with $ 2h_k\phi_3(h_k\mbf J_k)  \mvect D_{k}(\mvect X_{k1})$, so 
$\mvect X^{(2)}_{k1} = \mvect x_{k+1}^{(1)}$.
%\mvect x_k + h_k \mvect X_{1}^{(2)}(h_k) $
   \begin{eqnarray}   
         \Theta_3 \left(h ,\mvect d_{k,0} \right)  =  \frac{1}{h } \mbf T_k \mvect d_{k,0}    +   \frac{1}{h^2} \mbf T^2_k \mvect d_{k,0}    + \frac{1}{h^3} \left( e^{h \mbf J_k} -\mbf I_n   \right)\mbf T^3_k \mvect d_{k,0}   \nonumber  
   \end{eqnarray}
     % where
      %\begin{eqnarray}
      %$\mvect d_{k,i+1}    = \mbf T^2_k \mvect d_{k,0}  %\mvect d_{k,i} 
      %$. %\end{eqnarray}
%where $\mvect X^{(2)}_{3}$ denotes the operation in 2-stage for $\phi_3$ function and vector product.  
By reusing $\mvect x_{k+1}^{(1)}$,  the solution $\mvect x^{(2)}_{k+1}$ via 2-stage exponential Rosenbrock-Type method is
%\begin{eqnarray}
\begin{empheq}[box=\fbox]{align}
\mvect x^{(2)}_{k+1} % & = & % \mvect X_{k1}+   2h_k\phi_3(h_k\mbf J_k)  \mvect D_{k1}(\mvect X_{k1})  \nonumber \\
= x^{(1)}_{k+1}+ 2h_k \Theta_{3}(h_k,D_{k,0} (X^{(2)}_{k1}) %D_{k,2} (X^{(2)}_{k1}), D_{k,3} (X^{(2)}_{k1}))
)
% 2h_k\phi_3(h_k\mbf J_k)  \mvect D_{k1}(\mvect X_{k1})
\label{eq_2stage_final}
\end{empheq}
%\end{eqnarray}
 % \label{eq_rb_series}
 % \mvect D_{1} &=& \mvect D_{k1}(\mvect X_{k1}) \\
 % \mvect D_{2} &=& G^{-1}(\mvect x_k) \mbf C (\mvect x_k) \mvect D_{1} \\
 The error estimator becomes
%\begin{eqnarray}
$e^{(2)}_{rr} =   2h_k \Theta_{3}(h_k,D_{k,0} (X^{(2)}_{k1}))$.
%, D_{k,2} (X^{(2)}_{k1}), D_{k,3} (X^{(2)}_{k1}))
%\end{eqnarray}

\vspace{+0.08in}
\subsubsection{Three-stage exponential Rosenbrock-Type Formulation}  

Hochbruck, Ostermann, and Schweitzer \cite{Hochbruck09_RB} also designed the three-stage exponential Rosenbrock-Type method, which is,  
\begin{eqnarray}
\mvect X^{(3)}_{k1} &=& \mvect x_k+ \frac{1}{2}h_k \phi_1(\frac{1}{2}h_k \mbf J_k)\mvect g(\mbf x_k,\mvect u, t_k) +\left(\frac{1}{2}h_k \right)^2 \phi_2(\frac{1}{2}h_k \mbf J_k)\mvect b_k \nonumber\\
\mvect X^{(3)}_{k2} &=& \mvect x^{(1)}_{k+1}
%\mvect x_k+   h_k \phi_1( h_k \mbf J_k)\mvect g(\mbf x_k,\mvect u, t_k) 
%+ h_k^2 \phi_2(h_k \mbf J_k)\mvect b_k \nonumber\\  &+& 
% h_k^2 \phi_1( h_k \mbf J_k)\mvect g(\mbf x_k,\mvect u, t_k)+
+ h_k \phi_1(h_k \mbf J_k) \mvect D_{k}(\mvect X^{3}_{k1})  \nonumber\\
\mvect x_{k+1} &=& \mvect x_k+  h_k \phi_1( h_k \mbf J_k)\mvect g(\mbf x_k,\mvect u, t_k) + h_k^2 \phi_2( h_k \mbf J_k)\mvect b_k  \nonumber \\ 
&+& h_k (16\phi_3(h_k\mbf J_k) -48 \phi_4(h_k \mbf J_k)) \mvect D_{k}(\mvect X_{k1}) 
\nonumber \\
&+& h_k \left( -2\phi_3(h_k\mbf J_k) +12 \phi_4(h_k \mbf J_k)\right)  \mvect D_{k}(\mvect X_{k2})
\nonumber
 % \label{eq_rb_series}
\end{eqnarray}
The error estimator is
\begin{eqnarray}
 & & e^{(3)}_{rr}(\mvect x_{k+1}, \mvect X^{(3)}_{k2})   = \mvect x_{k+1} - \mvect X^{(3)}_{k2}  \nonumber \\ 
 & =    &
  h_k \left (16\phi_3(h_k\mbf J_k) -48 \phi_4(h_k \mbf J_k) - \phi_1(h_k \mbf J_k) \right) \mvect D_{k}(\mvect X^{(3)}_{k1})  \nonumber \\   
&+& h_k \left (-2\phi_3(h_k\mbf J_k) +12 \phi_4(h_k \mbf J_k) \right)  \mvect D_{k}(\mvect X^{(3)}_{k2})  %\nonumber \\ 
\end{eqnarray}
\begin{comment}

$e^{(3)}_{rr}(\mvect x_{k+1}, \mvect X^{(3)}_{k2})   = \mvect x_{k+1} - \mvect X^{(3)}_{k2}   
=
  h_k \left (16\phi_3(h_k\mbf J_k) -48 \phi_4(h_k \mbf J_k) - \phi_1(h_k \mbf J_k) \right) \mvect D_{k}(\mvect X^{(3)}_{k1})  \nonumber \\   
+ h_k \left (-2\phi_3(h_k\mbf J_k) +12 \phi_4(h_k \mbf J_k) \right)  \mvect D_{k}(\mvect X^{(3)}_{k2})$.  %\nonumber \\  

where 
\begin{eqnarray}
 \phi_4(h_k \mbf J_k) & = &  - \frac{1}{h_k} \left( \phi_3(h_k \mbf J_k) -\mbf I \right) \mbf G^{-1}(\mvect x_k) \mbf C (\mvect x_k)  \\
 & = &  \frac{1}{h_k^4} \left( e^{h_k \mbf J_k} -\mbf I   \right) 
 %\mbf G^{-1}(\mvect x_k) \mbf C (\mvect x_k)\mbf 
 \left( G^{-1}(\mvect x_k) \mbf C (\mvect x_k) \right)^4 
 \\
& +& \frac{1}{h_k^3}   \left( G^{-1}(\mvect x_k) \mbf C (\mvect x_k) \right)^3
 +   \frac{1}{h_k^2}    \left( G^{-1}(\mvect x_k) \mbf C (\mvect x_k) \right)^2 \nonumber  \\
  &+&   \frac{1}{h_k}    G^{-1}(\mvect x_k) \mbf C (\mvect x_k)  \nonumber  
 %\phi_3(h_n \mbf J_n) &=& - \frac{1}{h_n} (\phi_2(h_n \mbf J_n) -\frac{1}{2}\mbf I)\mbf G^{-1} \mbf C 
%\phi_3(h_n \mbf J_n) &=& - \frac{1}{h_n} (\phi_2(h_n \mbf J_n) -\frac{1}{2}\mbf I)\mbf G^{-1} \mbf C 
\end{eqnarray}
\end{comment}

The corresponding operations leading to final solution at 3-stage exponential Rosenbrock-Type method are %SPICE-like formulation:
\begin{eqnarray}
 \mvect X^{(3)}_{k1} =  \mvect x_k + \frac{h_k}{2} \Theta_1( \frac{h_k}{2}, \mvect x_{k,0}) +  \left( \frac{h_k}{2} \right)^2\Theta_{2}  ( \frac{h_k}{2},\mvect b_{k,0})
 %&=& \mvect x_k +   \left(e^{\frac{h_k}{2} \mbf J_k} -\mbf I \right) \mvect v_1   +   \left( e^{\frac{h_k}{2}\mbf J_k} -\mbf I \right)     \mvect v_{22}  +   \frac{h_k}{2}  \mvect v_{21}   
   \end{eqnarray}
   Note we do not need to update $\mvect v_{21}$ and $\mvect v_{22}$, since the slope during $[t_k,t_{k+1}]$ does not change.
   \begin{eqnarray}
   % \mvect X^{(3)}_{k1} = \mvect X^{(2)}_{k1},~~ 
       \mvect X^{(3)}_{k2} &=& \mvect x^{(1)}_{k+1} + h_k \mvect \Theta_{1}\left( h_k, \mvect D_1 (\mvect X_{k1}^{(3)})\right)
        \end{eqnarray}
         %+ \left(e^{h_k \mbf J_k} -\mbf I \right)  \mvect D_1 
     %\nonumber   \\ 
    %  \mvect X^{(3)}_{1} &=& \mvect X^{(2)}_{1} \\
      %\Theta_4(h ,\mvect d_1, \mvect d_2,\mvect d_3) &=& \frac{1}{h} \mvect d_1  -   \frac{1}{h^2} \mvect d_2  -  \frac{1}{h^3} \left( e^{h \mbf J_k} -\mbf I   \right) \mvect d_3  % \frac{1}{h_k } \mvect D^{(3)}_{31}  -   \frac{1}{h_k^2} \mvect D^{(3)}_{32}  -  \frac{1}{h_k^3} \left( e^{h_k \mbf J_k} -\mbf I   \right) \mvect D^{(3)}_{33} 
    %\nonumber   \\
%$\Theta_4$ operator is,
Then,
        \begin{eqnarray}   
         \Theta_4 \left(h ,\mvect d_{k,0} \right)  =  \frac{1}{h } \mbf T_k \mvect d_{k,0}    +   \frac{1}{h^2} \mbf T^2_k \mvect d_{k,0}  +    \frac{1}{h^3} \mbf T^3_k \mvect d_{k,0}   \nonumber \\  + \frac{1}{h^4} \left( e^{h \mbf J_k} -\mbf I_n   \right)\mbf T^4_k \mvect d_{k,0}   \nonumber  
   \end{eqnarray}
   The solution by 3-stage exponential Rosenbrock-Type method is
  \begin{empheq}[box=\fbox]{align}
 %\begin{eqnarray}
  % \mvect X_4^{(3)} &=& \frac{1}{h_k } \mvect D^{(3)}_{31}  +   \frac{1}{h_k^2} \mvect D^{(3)}_{32}  +   \frac{1}{h_k^4} \mvect D^{(3)}_{33} \\  &+& \frac{1}{h_k^4} \left( e^{h_k \mbf J_k} -\mbf I   \right) \mvect D^{(3)}_{34}  \\
 \mvect x^{(3)}_{k+1}  =  \mvect x^{(1)}_{k+1} + h_k \Theta_3 \left( h_k,D^{(16,-2)}_{3,0} \right)  %,D^{(16,-2)}_{3,2},D^{(16,-2)}_{3,3}
   + h_k \Theta_4 \left(h_k, D^{(-48,12)}_{4,0} \right)
 %, D^{(-48,12)}_{4,2},D^{(-48,12)}_{4,3}, D^{(-48,12)}_{4,4}
  \label{eq_3stage_final}
%\end{eqnarray}
\end{empheq}
where
%\begin{eqnarray}
$
\mvect D^{(16,-2)}_{k,0}(\mvect x_j)  =  %\left( \mbf G^{-1}(\mvect x_k) \mbf C(\mvect x_k) \right)   
  16 \mvect D_{k}(X^{(3)}_{k1}) - 2 \mvect D_{k}(X^{(3)}_{k2})$  and $   
%\mvect D^{(16,-2)}_{k,i+1}(\mvect x_j)   &=&  \left( -\mbf G^{-1}(\mvect x_k) \mbf C(\mvect x_k) \right)  \mvect D^{(16,-2)}_{k,i}(\mvect x_j)  
%\nonumber 
 %\\  
\mvect D^{(-48,12)}_{k,0}(\mvect x_j)   = % \left( \mbf G^{-1}(\mvect x_k) \mbf C(\mvect x_k) \right) ^{i-1}  
   12 \mvect D_{k}(X^{(3)}_{k2})-48 \mvect D_{k}(X^{(3)}_{k1})\nonumber $  % \\
%\mvect D^{(-48,12)}_{k,i+1}(\mvect x_j)   &=&  \left( -\mbf G^{-1}(\mvect x_k) \mbf C(\mvect x_k) \right)  \mvect D^{(-48,12)}_{k,i}  
%
%\end{eqnarray}

Then, the error estimation becomes
\begin{eqnarray}
e^{(3)}_{rr} =  h_k \left( \Theta_3 \left(h_k, \mvect D^{(3)}_{3,1} \right)  +  \Theta_4 \left(h_k, \mvect D^{(3)}_{4,0}   \right) \right) 
 - \Theta_1 \left(  h_k, \mvect D_{k}(\mvect X^{(3)}_{k1}) \right)
% \left(e^{h_k \mbf J_k} -\mbf I \right) \mvect D_{k1} 
\end{eqnarray}

\subsubsection{Summary}
Exponential Rosenbrock-Euler is the starting point kernel for the numerical integration. High-stage versions use higher order exponential functions, which we expect to gain faster Krylov convergence for subsequent projections \cite{Tokman10}.
Those internal stages of the above methods are just exponential Rosenbrock-Euler steps. 
This leads to simple methods that can be relatively cheaply implemented. 
%In comparison with Eq. (\ref{eq_rbe}) to obtain $\mvect x_{k+1}$, Eq. (\ref{eq_2stage_final}) requires extra MEVP of $  \left( e^{h_k \mbf J_k} -\mbf I   \right)  \mvect D_3 $, while Eq. (\ref{eq_3stage_final}) needs extra three MEVPs, such as $\left(e^{h_k \mbf J_k} -\mbf I \right)  \mvect D_1$, $\left( e^{h_k \mbf J_k} -\mbf I   \right) \mvect D^{(3)}_{33}$ and $ \left( e^{h_k \mbf J_k} -\mbf I   \right) \mvect D^{(3)}_{34}$, combined with more vector generation processes, e.g. $X^{(3)}_{k1}$, $\mvect D^{(3)}_{3i}$, $\mvect D^{(3)}_{4i}$.
%We exploit the choices for nonlinear circuit simulation, we found out ... 
%Another insight is the norm of $\mvect D_{kj}$ is usuage small, therfore, the Krylov subspace 

%=========================================================
\begin{comment}
To simplify the notation,
\begin{eqnarray}
\frac{d \mbf x(t)}{dt} - \mbf J \mbf x(t)  
 =  \mbf b(t)  + \mbf g_n(\mbf x)
\end{eqnarray}
where %The components for the above systems 
\begin{eqnarray}
\mbf J_n = -\mbf C^{-1} \mbf G , ~~
\frac{1}{\mbf J_n}=-\mbf G^{-1} \mbf C
\end{eqnarray}
%where %$\mbf C = \mbf C_l + \mbf C_{nl}$, $\mbf C_{nl}$ is the capactiance matrix from nonlinear devices.
%$\mbf G_{nl}$ is the conductance matrix from nonlinear devices.
The nonlinear effects are modeled as
\begin{eqnarray}
\mbf g_n(\mbf x_n) = \mbf C^{-1} \mbf I_{cur}(\mbf x_n) 
%, ~~\frac{1}{\mbf J_n}=-\mbf G^{-1} \mbf C
\end{eqnarray}
$F_n$ function is derived to meet Eq. (\ref{eq_rbeuler}).
\begin{eqnarray}
F_n(h_n \mbf J_n) = \mbf J_n \mbf x_n + \mbf g_n(\mbf x_n) + \mbf b(t_n) 
\end{eqnarray}
Then
\begin{eqnarray}
\phi_1(h_n \mbf J_n) &=& - \frac{1}{h_n} (e^{h_n \mbf J_n} -\mbf I)\mbf G^{-1} \mbf C  \\
\phi_2(h_n \mbf J_n) &=& - \frac{1}{h_n} (\phi_1(h_n \mbf J_n) -\mbf I)\mbf G^{-1} \mbf C  
%\phi_3(h_n \mbf J_n) &=& - \frac{1}{h_n} (\phi_2(h_n \mbf J_n) -\frac{1}{2}\mbf I)\mbf G^{-1} \mbf C 
\end{eqnarray}
The final equation are assembled as 
\begin{eqnarray}
& &  \mbf x_{n+1}  = \mbf x_n \\
   %\mbf x_n + (e^{h_n \mbf J_n} -\mbf I)(-\mbf G^{-1}) (-\mbf G \mbf x_n +  \mbf I_{cur}(\mbf x_n) +  \mbf Bu(t_n) ) 
  %	+  ( (e^{h_n\mbf J_n} -\mbf I)((\mbf G^{-1} \mbf C) - h_n  \mbf G^{-1} \mbf C )\mbf G^{-1} \mbf B  \frac{ \mbf u(t+h_n) - \mbf u(t)}{h_n} \nonumber  \\
 &+& (e^{h_n \mbf J_n} -\mbf I) 
           (\mbf x_n -  \mbf G^{-1}( \mbf I_{cur}(\mbf x_n) +  \mbf B \mbf u(t_n) ) ) \nonumber \\
   &+&  ( (e^{h_n\mbf J_n} -\mbf I) \mbf G^{-1} \mbf C\mbf G^{-1} \mbf B  \frac{ \mbf u(t+h_n) - \mbf u(t_n)}{h_n} \nonumber  \\
   &+ & h_n  \mbf G^{-1} \mbf C \mbf G^{-1} \mbf B  \frac{ \mbf u(t+h_n) - \mbf u(t_n)}{h_n} \nonumber   
\end{eqnarray} 
 There are two matrix exponential and vector products to evaluate $e^{h_n \mbf J_n} \mbf v_1
 $ and $e^{h_n\mbf J_n}\mbf v_2$ where 
 \begin{eqnarray}
 \label{eq_two_vec}
 \mbf v_1 =  \mbf x_n -  \mbf G^{-1}( \mbf I_{cur}(\mbf x_n) +  \mbf B \mbf u(t_n) ) 
 \nonumber 
 \\
 \mbf v_2 = \mbf G^{-1}\mbf C  \mbf G^{-1}\mbf B  \frac{ \mbf u(t+h_n) - \mbf u(t)}{h_n}
 \end{eqnarray}
 this leads to 
 \begin{eqnarray}
 \mbf x_{n+1}(h_n) & = & \mbf x_n - \mbf v1 - \mbf v2 
 %\nonumber \\
 %&+& \mbf G^{-1} \mbf C \mbf G^{-1} \mbf B  ( \mbf u(t+h_n) - \mbf u(t) ) \nonumber \\
 +  h_n \mbf v_2 \nonumber \\
 &+&  e^{h_n \mbf J_n}\mbf v_1 + e^{h_n \mbf J_n}\mbf v_2 
      \end{eqnarray}
 \end{comment}

%{\color{red}=============== stop here ============================}


==> emc14_abstract.tex <==
This paper proposes a matrix exponential time-integration based time-domain simulation algorithm for dynamic analysis of power delivery network (PDN) with nonlinear components. The proposed method is more efficient than traditional low order approximation methods, e.g. backward Euler method with Newton-Raphson iterations, in following aspects. First, the proposed method takes comparable number of time steps to complete the simulation, and solve the nonlinear PDN simulation problem using matrix exponential method. Second, the method takes only one LU decomposition per time step while backward Euler makes at least two LU decompositions. Moreover, our method does not need to repeat LU decomposition when we adjust the length of time steps for error controls. Third, the target matrix of our LU operation is much simpler, which is only conductance/resistance matrix. Since LU operation is very expensive during the large scale PDN simulation, such method is favored over the traditional algorithm framework when dealing with large scale problem. The experimental results validate our method's efficiency. In experimental results, we observe the reductions of total LU operation number and simulation runtime.


 
%Second, the invert Krylov space method inverses a much simpler matrix G than matrix G+C/h that is used by the backward Euler method. 
%Third, 

 
%Overall, we expect much more speedup for larger circuitry.

\begin{comment}
Time-domain circuit simulation using exponential method 
has many advantages, such as large time stepping,  stability. Previous,  matrix exponential-based methods \cite{Weng12_TCAD} \cite{Weng12_ICCAD} suffer the memory and runtime constraints from stiff circuit system. Those methods also require regularization to keep the storage element matrix non-singular. Above factors limit the scope of application. On the other hand, in current industry and academic, robust and standard method to solve general nonlinear circuit simulation is Newton-Raphson backward Euler method. However, it sometimes requires many iterations of solving linear system (e.g. LU solving) in order to satisfy the convergence condition as well as the truncation error budget. All degrade the performance of simulator.

In this work, we equip matrix exponential-based numerical integration kernel with exponential Rosenbrock-Euler method and Krylov subspace using inverted matrix bases. We remove the regularization process, reduce LU operations for each time stepping. We pose LU only on conductance/resistance matrix, which is much sparser than capacitance/inductance matrix after extraction. This property cannot be achieved non-matrix exponential-based integration kernels, due to the requirement of differential equation approximation. Therefore, such method can be much more robust for simulating strong parasitic cases. 
The experimental results show large speedups.
\end{comment}



==> intro.tex <==

Fast transient simulation with high accuracy has been a challenge in electronics design automation. 
In mainstream SPICE-like circuit simulators, a direct matrix solver with following backward forward substitution
are used for implicit linear multi-step schemes (backward Euler, trapezoidal, Gear's method, etc.)
Thanks to the recent developments in sparse matrix factorization techniques, 
such as KLU\cite{KLU2010}, NICSLU\cite{nicslu2013}, the direct methods have been applied to 
handle large-scale circuits. 

\begin{comment}
Power grid simulation is a very essential and computational heavy tasks during VLSI design.  
Given current stimulus and the power grid structure, 
designers could verify and predict the worst-case voltage noise 
through the simulation before signing off their design.  
However, with the huge size of modern design, power grid simulation is a time-consuming process. Moreover, manifesting effects 
from the package and the board would require longer simulation time, e.g., up to few $\mu s$, which worsens the performance 
of the power grid simulation. Therefore, an efficient power grid simulation is always a demand from industry. 

Conventionally, the power grid simulation is based on the trapezoidal method where the major computation is to solve a linear 
system by either iterative approaches or direct methods. 

%Many previous works~\cite{Chen01_Efficient}\cite{Feng08} 
%utilize iterative approaches to tackle 
%the scalability issue and enable adaptive stepping in the power grid simulation. 
The iterative methods usually suffer from the convergence problem 
because of the ill-conditioned matrix from the power grid design. On the other hand, the direct 
methods, i.e., Cholesky or LU factorizations, are more general for solving a linear system. Despite the huge memory 
demanding and computational effort, with a carefully chosen step size, the power grid simulation could perform only one 
factorization at the beginning while the rest of operations are just backward/forward substitutions. Since a power grid design 
usually includes board and package models, a long simulation time is required to manifest the low-frequency response. Hence, 
the cost of expensive factorization can be amortized by many faster backward/forward substitutions. Such general factorization 
and fixed step size strategy\cite{Xiong12}\cite{Yang12}\cite{Yu12}\cite{Zhao02} is widely adopted in industry. 
\end{comment}

However, the exsisting direct method is build on top of the traditional linear multi-step
(LMS) schemes, which based on relatively lower order polynomial approximation \cite{Leon75}. 
The allowable step size is usually small due to the local truncation error (LTE).  
The adaptive stepping induces matrices re-factorizations for the convergence to balance 
the LTE and step size. 

As an alternative to such LMS method, matrix exponential method is based on analytical solution
for ordinary differential equations (ODE). 
As long as the exponential term is calculated accurate enough. The time step can be arbitary large. 
Nonetheless, the direct computation of matrix exponential is quite expensive. 
People use Krylov subspace method to compute it. 
With increasing the dimension of Krylov subspace, we can obtain more accurate matrix exponential 
with respective to the time step size. 
The dimension of Krylov subspace can be viewed as ``order of accuracy'' in the counterpart of LMS method.
An promising property of it is this order can be tuned adaptively in MEXP. 
Meanwhile,
given a particular scheme of LMS method, the order is fixed. 
The way it reduces the error of approximation is via shrinking time step, 
which will bring matrix refactorizatin overhead.
%The matrix exponential method (MEXP) for the circuit simulation has better accuracy and adaptivity because of the 
%analytical formulation and 
Another feature of MEXP is the scaling invariant 
Krylov subspace approximation\cite{Weng11_ASICON}\cite{Weng12_TCAD}. 
It is important because even when we change the time step, 
we can still reuse the factorized matrices and leverage
futher computational advantages compared with LMS ones.
%Unlike the fixed step size strategy, MEXP could 
%dynamically adjust the step size to exploit the 
%low-frequency response of the power grid without expensive computation. 
%However, 
%the step size in MEXP is limited by the stiffness of circuit. This constraint would drag 
%the overall performance of MEXP for the power grid simulation. 
%In this work, we tailor MEXP using \emph{rational Krylov subspace} 
%for the power grid simulation with adaptive time stepping. 

Despite the above advantages, one problem, which still haunts the MEXP method,
is to simulate stiff circuits where time constants varies by orders of magnitude. 
When using standard Krylov subspace, it first captures these large magnitude
eigenvalues first in order to reduce interpolation error. 
For passive systems, e.g. circuit, all eigenvalues are negative, 
eigenvalues with small magnitudes are ones dominate the circuit behavior.
Therefore,
the property of standard Krylov subspace is not favored in circuit simulation.
Chen, \emph{et. al.}\cite{Chen2014_ASPDAC} proposed 
extended Krylov subspace to remedy this problem. 
Zhuang, \emph{et. al.} \cite{Zhuang2013_ASICON} devised 
rational Krylov subspace and efficient solves
stiff power grid circuit simulation. 

In this paper, 
we provide the rational Krylov subspace for linear circuit simulation 
with more rigorous numerical computation fundation.
We also give the scheme of choosing parameters in Krylov subspace 
and more robust error calculation, which is compatible with SPICE-like error budget.
Then Krylov subspace in 
\cite{Weng12_TCAD}, \cite{Chen2014_ASPDAC}, \cite{Zhuang2013_ASICON} 
are compared.
The rest of this paper is organized as follows. 
Section II introduces the general matrix exponential formulation for linear circuits. 
Section III presents Krylov subspace approximations for MEXP.
Section IV discusses the adaptive control in MEXP. 
Section VI shows the experimental results and Section VII concludes
this paper.


\begin{comment}
\vspace{+0.4in}
The rational Krylov subspace uses $(\mbf{I}-\gamma \mbf{A})^{-1}$ as the basis instead of $\mbf{A}$
used in the conventional Krylov 
subspaces, where $\mbf I$ is an identity matrix and $\gamma$ is a predefined parameter. The rational basis limits the spectrum of a circuit system, and emphasizes small magnitude eigenvalues, which are important to exponential function, so that the exponential of a matrix can be accurately approximated 
%even under a large step size. 
.
As a result, MEXP with rational Krylov subspace can enjoy benefits of the adaptivity and the accuracy of MEXP. 
Even though the rational Krylov subspace still needs 
to solve a linear system as the trapezoidal method does, MEXP can factorize the matrix only once and then constructs the rest of 
rational Krylov subspaces by backward/forward substitutions. Therefore, MEXP can utilize its capability of adaptivity to accelerate 
the simulation with the same kernel operations as the fixed step size strategy. Overall, our MEXP enables adaptive time stepping for the power grid simulation with only one LU factorization, and allows scaling large step size without compromising the accuracy. 
The experimental results demonstrate the effectiveness of MEXP with adaptive step size. The industrial power grid designs can be accelerated 17X on average compared to the trapezoidal method. 

The rest of paper is organized as follows. Section~\ref{sec:preliminary} presents the background of the power grid simulation and MEXP. 
Sections~\ref{sec:rational_krylov} and~\ref{sec:adaptive_step_control} show the theoretical foundation of the rational Krylov subspace 
and our adaptive step scheme for the power grid simulation, respectively.  Section~\ref{sec:exp_results} presents experimental results 
of several industrial power grid designs. Finally, Section~\ref{sec:conclusion} concludes 
this paper. 
\end{comment}



==> intro.v1.tex <==

Power grid simulation is a very essential and computational heavy tasks during VLSI design.  
Given current stimulus and the power grid structure, 
designers could verify and predict the worst-case voltage noise 
through the simulation before signing off their design.  
However, with the huge size of modern design, power grid simulation is a time-consuming process. Moreover, manifesting effects 
from the package and the board would require longer simulation time, e.g., up to few $\mu s$, which worsens the performance 
of the power grid simulation. Therefore, an efficient power grid simulation is always a demand from industry. 

Conventionally, the power grid simulation is based on the trapezoidal method where the major computation is to solve a linear 
system by either iterative approaches or direct methods. 
%Many previous works~\cite{Chen01_Efficient}\cite{Feng08} 
%utilize iterative approaches to tackle 
%the scalability issue and enable adaptive stepping in the power grid simulation. 
The iterative methods usually suffer from the convergence problem 
because of the ill-conditioned matrix from the power grid design. On the other hand, the direct 
methods, i.e., Cholesky or LU factorizations, are more general for solving a linear system. Despite the huge memory 
demanding and computational effort, with a carefully chosen step size, the power grid simulation could perform only one 
factorization at the beginning while the rest of operations are just backward/forward substitutions. Since a power grid design 
usually includes board and package models, a long simulation time is required to manifest the low-frequency response. Hence, 
the cost of expensive factorization can be amortized by many faster backward/forward substitutions. Such general factorization 
and fixed step size strategy\cite{Xiong12}\cite{Yang12}\cite{Yu12}\cite{Zhao02} is widely adopted in industry. 

The matrix exponential method (MEXP) for the circuit simulation has better accuracy and adaptivity because of the 
analytical formulation and the scaling invariant Krylov subspace approximation\cite{Weng11_ASICON}\cite{Weng12_TCAD}. 
Unlike the fixed step size strategy, MEXP could 
dynamically adjust the step size to exploit the low-frequency response of the power grid without expensive computation. 
However, 
the step size in MEXP is limited by the stiffness of circuit. This constraint would drag 
the overall performance of MEXP for the power grid simulation. 

In this work, we tailor MEXP using \emph{rational Krylov subspace} for the power grid simulation with adaptive time stepping. 
The rational Krylov subspace uses $(\mbf{I}-\gamma \mbf{A})^{-1}$ as the basis instead of $\mbf{A}$
used in the conventional Krylov 
subspaces, where $\mbf I$ is an identity matrix and $\gamma$ is a predefined parameter. The rational basis limits the spectrum of a circuit system, and emphasizes small magnitude eigenvalues, which are important to exponential function, so that the exponential of a matrix can be accurately approximated 
%even under a large step size. 
.
As a result, MEXP with rational Krylov subspace can enjoy benefits of the adaptivity and the accuracy of MEXP. 
Even though the rational Krylov subspace still needs 
to solve a linear system as the trapezoidal method does, MEXP can factorize the matrix only once and then constructs the rest of 
rational Krylov subspaces by backward/forward substitutions. Therefore, MEXP can utilize its capability of adaptivity to accelerate 
the simulation with the same kernel operations as the fixed step size strategy. Overall, our MEXP enables adaptive time stepping for the power grid simulation with only one LU factorization, and allows scaling large step size without compromising the accuracy. 
The experimental results demonstrate the effectiveness of MEXP with adaptive step size. The industrial power grid designs can be accelerated 17X on average compared to the trapezoidal method. 

The rest of paper is organized as follows. Section~\ref{sec:preliminary} presents the background of the power grid simulation and MEXP. 
Sections~\ref{sec:rational_krylov} and~\ref{sec:adaptive_step_control} show the theoretical foundation of the rational Krylov subspace 
and our adaptive step scheme for the power grid simulation, respectively.  Section~\ref{sec:exp_results} presents experimental results 
of several industrial power grid designs. Finally, Section~\ref{sec:conclusion} concludes 
this paper. 



==> introduction.tex <==
VLSI design verification relies on the dynamic analysis of power delivery network (PDN) to estimate power supply noises. 
Currently, PDN is often modeled as a large-scale linear circuit system with voltage supplies and time-varying current sources \cite{Zhao02, Nassif08_Power}. However, in order to obtain more accurate analysis of the modern PDN, 
we sometimes need to take nonlinear components into considerations, 
such as PDN with power gated transistors, voltage regulators \cite{Zeng10_DAC}. Therefore, the previous linear system and solving process are not suffice for the purpose. Besides, the scales of computational problems are beyond million or billion nodes, which make the simulation problem extremely time-consuming.
 

%Such circuit is extremely large,  which makes the corresponding simulation very time-consuming. 
Conventional dynamic time-domain PDN simulation has widely-accepted approach: first, it is based on linear system model; 
Then, time-consuming LU decompositions are usually computed at the very beginning by direct solvers \cite{Davis06}. Only relatively cheap pairs of forward and back substitutions are necessary at following fixed time steps \cite{Yang12, Yu12, Xiong12, Li12_Tau}, or adaptive stepping via matrix exponential method \cite{Zhuang14_DAC, Zhuang13_ASICON}.  
There are not matrix factorizations during the time advancing. 
Once nonlinear components connecting to the PDN are considered in the model, factorization operations are hardly excluded.  
%is to first factorize matrix, then utilize fixed time step to run through %the time domain simulation via forward and backward substations.   
The previous procedure of solving nonlinear system requires Newton-Raphson iterations for each time step, where at least two LU decompositions are involved, till the solutions are converged. 
Besides, in PDN simulation, long time span/large number of time steps always accompanies with such time-consuming LU operations. 
Therefore, it is crucial to devise efficient PDN simulation algorithms by reducing expensive LU operations, increasing time step-sizes, while maintaining high accuracy.
% for PDN with nonlinear components. 

The problems of conventional methods come from they are based on low order implicit approximations of differential equations, such as backward Euler method, trapezoidal method, for time-integrations. There are several drawbacks as follows. 
First, the local truncation error (LTE) is in positive proportion to time step size. The time step size cannot be very large. 
Second, such low order approximation requires time step embedded in the linear matrix formulation for matrix factorizations.
Once the time steps are adjusted,  LU decompositions are unavoidable. 
Beyond those low order approximation strategies, matrix exponential time-integration kernel has  been applied for nonlinear circuit simulation \cite{Weng12_TCAD, Weng12_ICCAD}. This kernel has better properties of accuracy and time-step controlling.
It has high order approximation for differential equations. 
Moreover, it does not embed time step size in matrix, which is the target of LU decompositions.  
The drawbacks of previous works are the slow convergence rates for matrix exponential and vector product (MEVP) by Krylov subspace \cite{Zhuang14_DAC}.  
The nonlinear circuit formulation still costs many LU operations to converge the solutions \cite{Weng12_TCAD}. 

In this work, we design one-stage exponential Rosenbrock-Euler method \cite{Caliari09_ER, Hochbruck09_RB, Carr13}, which is still based on matrix exponential time-integration kernel. The MEVP is computed via inverted Krylov subspace \cite{Zhuang14_DAC}.
{\bf {The contributions}} of this paper are as follows. 
\begin{itemize}
\item The proposed method takes only one LU decomposition per time step while conventional Newton-Raphson backward Euler method requires at least two operations.
\item Moreover, proposed method does not need to repeat LU decomposition when we adjust the length of time steps for error controls.
\item The proposed method manages to complete the simulation using less time steps due to better precision and longer time steps by the matrix exponential kernel. 
\item Besides, the proposed method avoids costly regularization process \cite{Weng12_TCAD, Chen12_TCAD}.
\end{itemize}

The remainder of this paper is organized as follows. Section II introduces the background of circuit simulation. Section III presents the exponential Rosenbrock-Euler method. Section IV illustrates Krylov subspace method to approximate MEVP using inverted bases. Section V shows the experimental results. Section VI concludes this paper. 
%Besides,we also overcome above problems for matrix exponential-based integration kernel by changing Krylov subspace using inverted bases, inspired by the work \cite{Zhuang14_DAC}. 
%Another outstanding property of inverted bases is it needs only   conductance/resistance matrix factorization.
%When the existence of strong coupling, the capacitance/inductance matrix would be much denser. 
%For example, when the accuracy is demanded we lowering threshold to extract the parastics \cite{Yu2013}\cite{Zhuang2012}, there will be more and more elements in $\mbf C$ matrix with large value ranges. 
%This property is a very good candidate to handle such problem and it cannot be achieved within the framework of traditional time-differencing methods. The factorization always accompanies with capacitance/inductance matrix. 









\begin{comment}
Time-domain simulation involes solving differntial equations, which describes the behavior of circuit. The traditional ways to approximate differential equations (time-differencing) are backward Euler, trapezoidal, and Gear's method. Backward Euler method has good stability, which are used in most of circuit simulators and served as baseline method. %\emph{de factor}.  
In general nonlinear circuit simulation, each time step requires several Newton-Raphson iterations. After iterations, the local truncation error (LTE) from certain time-differencing strategy 
should be also checked and ensured below  error budget. If the condition is violated, the circuit simulator need to perform new Newton-Raphson iterations with smaller time step until the LTE estimation is satisfied.
The whole process contains a large number of  matrix solving operations, of which is time-consuming when the circuit system contains huge number of unkowns. 

 
Apart from traditional time-differencing approximation, matrix exponential based time integration triggers new research interests in time-domain simulation \cite{Weng12_TCAD} \cite{Weng12_ICCAD} \cite{Zhuang13_ASICON} \cite{Zhuang14_DAC} \cite{Zhuang15_DAC_NL} \cite{Zhuang15_DAC_PowerSnap}. 
In this method, the step size is free from restrictions of the stability and the LTE of polynomial expansion. Despite such nice property, the matrix exponential is expensive so that Krylov subspace is utilized to approximate matrix exponential-and-vector product (MEVP) $e^{\mbf A}\mbf v$. The Krylov subspace method used by Weng \emph{et. al.} \cite{Weng12_TCAD} \cite{Weng12_ICCAD} consumes large amount of memory to build bases for MEVP when circuit system is stiff (the values in the matrices vary in large magnitude, such as the existence of small and large capacitances). It also requires regularization of capacitance/inductance matrix to remove singularity. Those all degrades runtime and memory performance for circuit simulation solver.
\end{comment}


==> sub-concl.tex <==





Excellent Krylov Subspace for MEXP.

Better Error evaluation. SPICE-like.

$\gamma $ choice




==> sub-concl.v1.tex <==
For large scale power grid simulation, we propose an MEXP framework using two methods 
rational Krylov subspace approximation and adaptive time stepping technique. 
The former method can relax stiffness constraint of~\cite{Weng11_ASICON}\cite{Weng12_TCAD}. 
The later one helps adaptively exploit low-, mid-, and high-frequency property in   
simulation of industrial PDN designs.
In the time-consuming impulse response simulation, the proposed method 
achieve more than 15 times speedup on average over the widely-adopted fixed-step trapezoidal method. 



==> sub-exp_results.tex <==

We prototype MEXP with different Krylov subspace in MATLAB. Experiement are performance on  
XXX GHz CPU and XX GB memory, with testbench circuits of different sizes and characteristics.


Table \ref{tab:linear_designs} provides detailed specifications. Type indicates linear. 
Index gives the DAE index of the MNA systems. 
The numbers of nonzeros in C + G
before and after regularization are also shown. For fairness,
a MATLAB implementation of TRAP is used to provide
benchmarks for accuracy and performance comparisons. All
linear systems are solved by the direct solver (backslash) in
MATLAB.



\subsection{R-MEXP with $\gamma$ choice}

\subsection{Error Evaluation}

\subsection{Performance of Fixed Time Step MEXPs}

{\color{red} rerun the test using new error term}

\begin{table}[ht]
    \caption{Comparisions among MEXP, I-MEXP and R-MATEX with RC cases}
    \centering
    \begin{tabular}{|c||c|c|c|c|c|c|}
    \hline
	Method  & $m_{a}$ &   $m_{p} $  & Err(\%)    & Spdp 
	& {Stiffness}  \\ 
	\hline
	MEXP	&  211.4   	&   229  	&  0.510   & -- &
	\multirow{3}{*}{$2.1 \times 10^{16}$ } 
	\\
	\cline{1-5}
	I-MEXP	& 5.7 	&14       &  0.004	   & 2616X   &   \\
	\cline{1-5}
	E-MEXP	&   	&       &  	   &    &   \\
	\cline{1-5}
	R-MEXP	& 6.9   & 12   &  0.004   &  2735X   & \\ 
	\hline
	\hline
	MEXP	&  154.2   	&   224  	&  0.004 & --  
	& 	    \multirow{3}{*}{$2.1 \times 10^{12}$ } 
	\\
	\cline{1-5}
	I-MEXP	&  5.7 	& 14       &0.004   &  583X  &   \\
	\cline{1-5}
	E-MEXP	&   	&       &  	   &    &   \\
	\cline{1-5}
	R-MEXP	& 6.9  & 12   &  0.004 	   &  611X  & \\ 
	\hline
	\hline
	MEXP &  148.6   	&   223  & 0.004  &  -- & 	    \multirow{3}{*}{$2.1 \times 10^{8}$ } 
	\\
	\cline{1-5}
	I-MEXP	& 5.7  	& 14      & 0.004     & 229X  &   \\
	\cline{1-5}
	E-MEXP	&   	&       &  	   &    &   \\
	\cline{1-5}
	R-MEXP	& 6.9  & 12   &  0.004  &  252X  & \\ 
	%\cline{1-6}
	\hline
    \end{tabular}
    \label{tab:rc_ckt}
\end{table}

\subsection{Performance of Adaptive MEXPs}

\begin{table*}[htp]
    \caption{Specifications of Linear Circuit Designs}
    \centering
    \begin{tabular}{|c||r|r|r|r|}
    \hline
	Design   	& \multicolumn{1}{|c|}{\#R}	    
		       	& \multicolumn{1}{|c|}{\#C}	
		       	& \multicolumn{1}{|c|}{\#L}	    
		       	& \multicolumn{1}{|c|}{\#Nodes}  \\ \hline
	D1	 	& 23221	    & 15193	& 15193	    & 45.7K	\\ \hline
	D2	   	& 348582    & 228952	& 228952    & 688K	\\ \hline
	D3	   	& 1468863   & 965540	& 965540    & 2.90M	\\ \hline
	D4	   	& 3748974   & 2467400	& 2464819   & 7.40M	\\ 
    \hline
    \end{tabular}
    \label{tab:linear_designs}
\end{table*}




==> sub-exp_results.v1.tex <==

In this section, we compare performance of the power grid simulation 
by MEXP and the trapezoidal method (TR).
MEXP with adaptive step size control follows Algorithm~\ref{algo:adaptive_step}. 
We predefine $\gamma$ e.g. $10^{-10}$ here. 
and restrict the maximum allowed step size within $1ns$ to have enough time instants to plot the figure.
It is possible to have more fine-grain time instants, e.g., $10ps$, with only negligible cost by adjusting 
$\alpha$ in Eqn. (\ref{eq:scale}). TR is in fixed step size $h$ in order to minimize the cost 
of LU factorization. Both methods only perform factorization once for transient simulation, 
and rest of operations is mainly backward/forward 
substitution. We implement both methods in MATLAB and use UMFPACK package for LU factorization. Note that even 
though previous works\cite{Chen01_Efficient}\cite{Su03} show that using iterative 
approach in TR 
could also achieve adaptive step control, 
long simulation time span in power grid designs make direct 
method with fixed step size more desirable\cite{Xiong12}\cite{Yang12}\cite{Zhao02}. 
The experiments are performed on a Linux workstation with an Intel Core i7-920 2.67GHz CPU and 12GB memory.
The power grid consists of four metal 
layers: M1, M3, M6 and RDL. The physical parameters of each metal layer is listed in Table~\ref{tab:spec_metal_layers}. 
The package is modeled as an RL series at each C4 bump, and the board is modeled as a lumped RLC network. The
specification of each PDN design is listed in Table~\ref{tab:spec_pdn_designs} where the size of each design 
ranges from $45.7$K to $7.40$M. 
\vspace{-0.1in}
\begin{table}[htp]
  \caption{Widths and pitches of metal layers in the PDN design($\mu m$).}
  \centering
  \begin{tabular}{cccccccc}
    \multicolumn{2}{c}{M1} &\multicolumn{2}{c}{M3} &\multicolumn{2}{c}{M6} &\multicolumn{2}{c}{RDL}\\
    \hline pitch &width  &pitch &width  &pitch &width  &pitch &width \\
    \hline 2.5   &0.2  &8.5  &0.25  &30 &4 &400 &30\\
    \hline 
  \end{tabular}
  \label{tab:spec_metal_layers}
\end{table}
\vspace{-0.2in}
\begin{table}[htp]
    \caption{Specifications of PDN Designs}
    \centering
    \begin{tabular}{|c||c|r|r|r|r|}
    \hline
	Design  & Area ($mm^2$)	& \multicolumn{1}{|c|}{\#R}	    
				& \multicolumn{1}{|c|}{\#C}	
				& \multicolumn{1}{|c|}{\#L}	    
				& \multicolumn{1}{|c|}{\#Nodes}  \\ \hline
	D1	& $0.35^2$	& 23221	    & 15193	& 15193	    & 45.7K	\\ \hline
	D2	& $1.40^2$  	& 348582    & 228952	& 228952    & 688K	\\ \hline
	D3	& $2.80^2$  	& 1468863   & 965540	& 965540    & 2.90M	\\ \hline
	D4	& $5.00^2$  	& 3748974   & 2467400	& 2464819   & 7.40M	\\ 
    \hline
    \end{tabular}
    \label{tab:spec_pdn_designs}
\end{table}
\vspace{-0.1in}

In order to characterize a PDN design, designers can rely on the simulation result of impulse response of the 
PDN design. Many previous works\cite{Du10}\cite{Tian96} have proposed different PDN analysis based on the impulse 
response. The nature of impulse response of the PDN design, which contains low-, mid- and high-frequency components, 
can significantly enjoy the adaptive step size in MEXP.  We would also like to mention that the impulse response 
based analysis is not only for the PDN design, but also for worst-case eye opening analysis in the high speed interconnect
%\cite{Analui05}
\cite{Shi08}. 

The impulse response can be derived from the simulation result of a step input from $0$V to $1$V with a small transition
time. Hence, we inject a step input to each PDN design and compare the performance of MEXP and TR. The transition time of 
the step input and the simulation time span is $10ps$ and $1\mu s$ for observing both high- and low-frequency responses. 
Table~\ref{tab:results_pdn_cases} shows the simulation runtime of MEXP and TR where the fixed step size is set as $10ps$ 
to comply with the transition time. In the table, ``DC'', ``LU'' and ``Time'' indicate the runtime for DC analysis, LU 
factorization and the overall simulation, respectively. DC analysis is also via the LU factorization. We can also adopt 
other techniques\cite{Xiong12}\cite{Yang12}\cite{Yu12} to improve the performance of DC analysis for both methods. 
%The test cases include different industrial power distribution networks (PDNs), 
%%which contain on-chip power grid, the model of 
%board and package. 
It is noted that these cases are very stiff and 
with singular matrix $\mbf C$. 
We do not use the method\cite{Weng11_ASICON}\cite{Weng12_TCAD} on the benchmarks, 
because that it cannot
handle the singular $\mbf C$ in 
these industrial PDN design
without regularization.
It is worth pointing out that
even after regularization\cite{Weng12_TCAD}, the stiffness still causes large  $m$ series for matrix
exponential evaluation.
For example, we construct a simple RC mesh network with 2500 nodes. 
The extreme values of this circuit are 
$\mbf C_{min}=5.04 \times 10^{-19}$,
$\mbf C_{max}=1.00 \times 10^{-15}$,
$\mbf G_{min}=1.09 \times 10^{-2}$, 
and $\mbf G_{max}=1.00 \times 10^2$. 
The corresponding maximum eigenvalue 
of $-\mbf C^{-1}\mbf G$ is $-1.88 \times 10^{9}$
and minimum eigenvalue is $-3.98 \times 10^{17}$. 
The stiffness is 
$ \frac{Re(\lambda_{min})}{Re(\lambda_{max})}= 2.12 \times 10^{8}$ .
During simulation of $1ns$ time span, with a fixed step size $10ps$, MEXP based on~\cite{Weng11_ASICON}\cite{Weng12_TCAD} costs 
average and peak dimensions of Krylov subspace $m_{avg}$ = 115, and
$m_{peak}$=264, respectively. 
Our MEXP uses rational Krylov subspaces, which only need $m_{avg}$=3.11, $m_{peak}$=10
and lead to 224X speedup in total runtime.
%``Spdp'' shows the speedup of MEXP over TR. 

In these test cases, our MEXP has significant speedup over TR because it can
adaptively exploit much large step size to simulate the design whereas TR can 
only march with $10ps$ time step for whole $1\mu s$ time span. The average speedup is 17X.  Fig.~\ref{fig:result_pdn_case1} shows the 
simulation result of design D1 at a node on M1. As we can see, the result by MEXP and TR are very close to the result of 
HSPICE, which is as our reference result here. The errors of MEXP and TR to HSPICE are $7.33\times10^{-4}$ and $7.47\times10^{-4}$.  
This figure also demonstrates that a PDN design has low-, mid- and high-freqeuncy 
response so that long simulation time span is necessary, meanwhile, small time steps are required during the 20$ns$ in the beginning. 
\vspace{-0.1in}
\begin{table}[htp]
    \centering
    \caption{Simulation runtime of PDN designs}
    \begin{tabular}{|c||r||r|r||r|r|r|}
    \hline
	\multirow{2}{*}{Design} & \multirow{2}{*}{DC(s)} &\multicolumn{2}{c||}{TR ($h=10ps$)} & \multicolumn{3}{c|}{Our MEXP ($\gamma=10^{-10}$) }  \\ 
	\cline{3-7} 
				 &	  &\multicolumn{1}{|c|}{LU(s)}   
					  &\multicolumn{1}{|c||}{Total}	
					  &\multicolumn{1}{|c|}{LU(s)}	 
					  &\multicolumn{1}{|c|}{Total}		
					  &\multicolumn{1}{|c|}{Speedup}  \\ \hline
        D1			 &0.710	  &0.670	   &44.9m	&0.680	 &2.86m		& 15.7 \\ \hline
        D2 			 &12.2	  &15.6  &15.4h	&15.5	 &54.6m	& 16.9 \\ \hline
        D3 			 &69.6   &91.6   &76.9h	&93.3	 &4.30h		& 17.9 \\ \hline
        D4 			 &219  &294  &204h	&299	 &11.3h	& 18.1	\\ 
    \hline
    \end{tabular}
    \label{tab:results_pdn_cases}
\end{table}
\begin{figure}[ht]
    \centering
    \includegraphics[width=3.3in]{./figs/result_pdn_case1.eps}
    \caption{Result of D1}
    \label{fig:result_pdn_case1}
\end{figure}




==> sub-exp_results.v2.tex <==

\begin{comment}
\end{comment}
We prototype MEXP with different Krylov subspace in MATLAB. Experiement are performance on  
XXX GHz CPU and XX GB memory, with testbench circuits of different sizes and characteristics.

Table \ref{} provides detailed specifications. Type indicates linear
(L) or nonlinear (NL) circuits. Index gives the DAE index
of the MNA systems. The numbers of nonzeros in C + G
before and after regularization are also shown. For fairness,
a MATLAB implementation of TRAP is used to provide
benchmarks for accuracy and performance comparisons. All
linear systems are solved by the direct solver (backslash) in
MATLAB.

\vspace{-0.1in}
\begin{table}[htp]
  \caption{Widths and pitches of metal layers in the PDN design($\mu m$).}
  \centering
  \begin{tabular}{cccccccc}
    \multicolumn{2}{c}{M1} &\multicolumn{2}{c}{M3} &\multicolumn{2}{c}{M6} &\multicolumn{2}{c}{RDL}\\
    \hline pitch &width  &pitch &width  &pitch &width  &pitch &width \\
    \hline 2.5   &0.2  &8.5  &0.25  &30 &4 &400 &30\\
    \hline 
  \end{tabular}
  \label{tab:spec_metal_layers}
\end{table}
\vspace{-0.2in}
\begin{table}[htp]
    \caption{Specifications of PDN Designs}
    \centering
    \begin{tabular}{|c||c|r|r|r|r|}
    \hline
	Design  & Area ($mm^2$)	& \multicolumn{1}{|c|}{\#R}	    
				& \multicolumn{1}{|c|}{\#C}	
				& \multicolumn{1}{|c|}{\#L}	    
				& \multicolumn{1}{|c|}{\#Nodes}  \\ \hline
	D1	& $0.35^2$	& 23221	    & 15193	& 15193	    & 45.7K	\\ \hline
	D2	& $1.40^2$  	& 348582    & 228952	& 228952    & 688K	\\ \hline
	D3	& $2.80^2$  	& 1468863   & 965540	& 965540    & 2.90M	\\ \hline
	D4	& $5.00^2$  	& 3748974   & 2467400	& 2464819   & 7.40M	\\ 
    \hline
    \end{tabular}
    \label{tab:spec_pdn_designs}
\end{table}
\vspace{-0.1in}

In order to characterize a PDN design, designers can rely on the simulation result of impulse response of the 
PDN design. Many previous works\cite{Du10}\cite{Tian96} have proposed different PDN analysis based on the impulse 
response. The nature of impulse response of the PDN design, which contains low-, mid- and high-frequency components, 
can significantly enjoy the adaptive step size in MEXP.  We would also like to mention that the impulse response 
based analysis is not only for the PDN design, but also for worst-case eye opening analysis in the high speed interconnect
%\cite{Analui05}
\cite{Shi08}. 

The impulse response can be derived from the simulation result of a step input from $0$V to $1$V with a small transition
time. Hence, we inject a step input to each PDN design and compare the performance of MEXP and TR. The transition time of 
the step input and the simulation time span is $10ps$ and $1\mu s$ for observing both high- and low-frequency responses. 
Table~\ref{tab:results_pdn_cases} shows the simulation runtime of MEXP and TR where the fixed step size is set as $10ps$ 
to comply with the transition time. In the table, ``DC'', ``LU'' and ``Time'' indicate the runtime for DC analysis, LU 
factorization and the overall simulation, respectively. DC analysis is also via the LU factorization. We can also adopt 
other techniques\cite{Xiong12}\cite{Yang12}\cite{Yu12} to improve the performance of DC analysis for both methods. 
%The test cases include different industrial power distribution networks (PDNs), 
%%which contain on-chip power grid, the model of 
%board and package. 
It is noted that these cases are very stiff and 
with singular matrix $\mbf C$. 
We do not use the method\cite{Weng11_ASICON}\cite{Weng12_TCAD} on the benchmarks, 
because that it cannot
handle the singular $\mbf C$ in 
these industrial PDN design
without regularization.
It is worth pointing out that
even after regularization\cite{Weng12_TCAD}, the stiffness still causes large  $m$ series for matrix
exponential evaluation.
For example, we construct a simple RC mesh network with 2500 nodes. 
The extreme values of this circuit are 
$\mbf C_{min}=5.04 \times 10^{-19}$,
$\mbf C_{max}=1.00 \times 10^{-15}$,
$\mbf G_{min}=1.09 \times 10^{-2}$, 
and $\mbf G_{max}=1.00 \times 10^2$. 
The corresponding maximum eigenvalue 
of $-\mbf C^{-1}\mbf G$ is $-1.88 \times 10^{9}$
and minimum eigenvalue is $-3.98 \times 10^{17}$. 
The stiffness is 
$ \frac{Re(\lambda_{min})}{Re(\lambda_{max})}= 2.12 \times 10^{8}$ .
During simulation of $1ns$ time span, with a fixed step size $10ps$, MEXP based on~\cite{Weng11_ASICON}\cite{Weng12_TCAD} costs 
average and peak dimensions of Krylov subspace $m_{avg}$ = 115, and
$m_{peak}$=264, respectively. 
Our MEXP uses rational Krylov subspaces, which only need $m_{avg}$=3.11, $m_{peak}$=10
and lead to 224X speedup in total runtime.
%``Spdp'' shows the speedup of MEXP over TR. 

In these test cases, our MEXP has significant speedup over TR because it can
adaptively exploit much large step size to simulate the design whereas TR can 
only march with $10ps$ time step for whole $1\mu s$ time span. The average speedup is 17X.  Fig.~\ref{fig:result_pdn_case1} shows the 
simulation result of design D1 at a node on M1. As we can see, the result by MEXP and TR are very close to the result of 
HSPICE, which is as our reference result here. The errors of MEXP and TR to HSPICE are $7.33\times10^{-4}$ and $7.47\times10^{-4}$.  
This figure also demonstrates that a PDN design has low-, mid- and high-freqeuncy 
response so that long simulation time span is necessary, meanwhile, small time steps are required during the 20$ns$ in the beginning. 
\vspace{-0.1in}
\begin{table}[htp]
    \centering
    \caption{Simulation runtime of PDN designs}
    \begin{tabular}{|c||r||r|r||r|r|r|}
    \hline
	\multirow{2}{*}{Design} & \multirow{2}{*}{DC(s)} &\multicolumn{2}{c||}{TR ($h=10ps$)} & \multicolumn{3}{c|}{Our MEXP ($\gamma=10^{-10}$) }  \\ 
	\cline{3-7} 
				 &	  &\multicolumn{1}{|c|}{LU(s)}   
					  &\multicolumn{1}{|c||}{Total}	
					  &\multicolumn{1}{|c|}{LU(s)}	 
					  &\multicolumn{1}{|c|}{Total}		
					  &\multicolumn{1}{|c|}{Speedup}  \\ \hline
        D1			 &0.710	  &0.670	   &44.9m	&0.680	 &2.86m		& 15.7 \\ \hline
        D2 			 &12.2	  &15.6  &15.4h	&15.5	 &54.6m	& 16.9 \\ \hline
        D3 			 &69.6   &91.6   &76.9h	&93.3	 &4.30h		& 17.9 \\ \hline
        D4 			 &219  &294  &204h	&299	 &11.3h	& 18.1	\\ 
    \hline
    \end{tabular}
    \label{tab:results_pdn_cases}
\end{table}
\begin{figure}[ht]
    \centering
    \includegraphics[width=3.3in]{./figs/result_pdn_case1.eps}
    \caption{Result of D1}
    \label{fig:result_pdn_case1}
\end{figure}




==> sub-krylov_approx.tex <==

\subsection{Matrix Exponential Computation using Standard Krylov Subspace (S-MEXP)}

The computation of the matrix exponential 
\begin{eqnarray}
\label{eq:exp_taylor}
e^{\mbf A}\mbf v:=  \mbf {(I + A + \frac{A^2}{2!} + ... +\frac{ A^{n-1}}{k!}+...)v}. 
\end{eqnarray}
is extremely expensive.  
Thanks to well-known Krylov subspace algorithm~\cite{Weng12_TCAD, Weng12_ICCAD, Hochbruck97, Saad92}. 

The Krylov subspace spans by the basis of $m$ vector
 \begin{eqnarray}
\label{eq:kryspan}
{\rm K_m}\left(\mbf{A}, \mbf{v}\right) := span\{\mbf {v, Av, A^2v, ..., A^{n-1}v}\}. 
\end{eqnarray}
Generally, the orthogonal bases of Krylov subspace can be constructed from Arnoldi or Lanczos process. 
 \begin{eqnarray}
\label{eq:kryspan}
\mbf {AV_m} =  \mbf {V_mH_m+H}(m+1,m)\mbf {v_{m+1}e^T_m}
\end{eqnarray}
where $\mbf{H_m}$ is Hessenberg matrix, $\mbf e_m$ is the $m$th unit vector with dimension $m \times 1$.
Assume $ \mbf {V^{T}_mAV_m =  H_m }$.
Therefore, $e^{\mbf{A}}\mbf{v}$ can be projected onto the Krylov 
subspace ${\rm K_m}\left(\mbf{A}, \mbf{v}\right)$ with dimension of $m$. 
Then~(\ref{eq:exp_taylor}) is evaluated by 
\begin{eqnarray}
\label{eq:Krylov_exp}
e^{\mbf A} \mbf v  \approx
 \mbf {V_m} \mbf {V^T_m}  e^{\mbf A} \mbf {V_m}  \mbf {V^T_m v}  = || \mbf v || \mbf {V_m} e^{\mbf H_m} \mbf e_1 
\end{eqnarray}


The convenient posterior error estimation is used for matrix exponential and vector product as follows,

\begin{eqnarray}
r_m(h) = \left\| v \right\| \left  | e_m^{\mathsf{T}} e^{h \mbf H_m } e_1 \right |
\end{eqnarray}


It is noted that in experiment for circuit simulation, the order $m$ is usually small, the overall computational complexity of exponential operator is greately reduce, so the scalability of MEXP is better than traditional implicit methods. 
The works in~\cite{Weng12_TCAD, Weng12_ICCAD}
 use $\mbf{C}^{-1}(\mbf{G}\mbf{v})$ 
instead of computing $\mbf{C}^{-1}$ explicitly. 
These works claim solving $\mbf{C}$ is easier than $(\mbf{C}/h+\mbf{G})$ of implicit methods 
because $\mbf{C}$ has 
fewer non-zeros and better structure that can favor direct and iterative sparse solvers. 
However, if the circuit system is stiff or even singular $w.r.t.$ $\mbf C$, which will hamper the efficiency of calculation.
The Krylov subspace method, using matrix $\mbf A$ directly to form the bases, needs a large $m$ 
or a small $h$ to provide sufficient resolution 
to the spectrum of $\mbf{A}h$. Besides that, the large storage of $m$ bases for the high stiffness limits the size of circuit. 
We will address the issue in the following section using different basis
for Krylov subspace methods.

\begin{algorithm}
\label{algo:arnoldi_std}
\caption{Arnoldi process in MEXP with Standard Krylov Subspace}
%$\rm K_m(\mbf X_1^{-1}\mbf X_2, \mbf v)$} %~\cite{Weng12_TCAD, Weng12_ICCAD}}
\KwIn{ $\mbf L, \mbf U, \mbf G, h ,\mbf x(t),  \epsilon $  }
%\KwOut{ $\mbf V_m, \mbf H_m,  m$ }
\KwOut{ $\mbf x(t+h)$ }
    {   
%	[$\mbf L, \mbf U$]=LU($\mbf X_1$)\\
%	Normalize the intial vector 
	$\mbf v = \mbf x(t), \mbf v_1 = \frac{\mbf v }{\lVert \mbf v \rVert}$\;
	\For  {$j=1:m$}
	{
	   % Calculate 
%	    $   \mbf w =  \mbf X_1^{-1} \mbf X_2 \mbf v_{j} $ by solving
	    $\mbf w = \mbf U^{-1}  (\mbf L^{-1} (\mbf G \mbf v_{j})) $ \;
	    \For {$i = 1:j$}
	    {
	%	Orthogonalization 
		$h_{i,j} = \mbf w^T\mbf v_{j}$\;
		$\mbf w = \mbf w - h_{i,j} \mbf v_{j}$\;
	    }
	    $h_{j+1,j} = \lVert \mbf w \rVert $\;
	    $\mbf v_{j+1} = \frac{\mbf w }{h_{j+1,j}} $\;
	    % \If {$ h_{i+1,j} < \epsilon $}
	    \If {$ || \mbf r_j(h)|| < \epsilon $}
	    {
		$m = j$\;
		break\;
	    }
	}
	$\mbf x(t) = \lVert \mbf v \rVert \mbf {V_m} e^{h \mbf H_m} \mbf e_1 $\;
	%$\lVert r_m(h) \rVert  =  \lVert \mbf v \rVert \left| h_{m+1,m} e_m^T e^{h\mbf H_m} e_1 \right|$
    }
\end{algorithm}

 
\subsection{Matrix Exponential Computation by Inverted Krylov Subspace Basis (I-MEXP)}

%Based on the rationale that standard Krylov subspace method
%tends to approximate large magnitude eigenvalues of $\mbf A$. 
%Then, 
The standard Krylov subspace prioritize the approximation of large magnitude eigenvalues, which is correspondingly the fast modes in the circuit. However, 
designers are more focus on the slow mode, due to the fast mode dies down very quickly and slow mode shapes the behavior of circuit.

Then, instead of $\mbf A$, we use $\mbf A^{-1}$ (or say, $\mbf G^{-1} \mbf C$) as our target matrix, %then recover it 
\begin{eqnarray}
{\rm K_m}(\mbf A^{-1} , v) := \text{span}
{\{ \mbf v, \mbf A^{-1}\mbf v, \cdots, \mbf A^{-(m-1)} \mbf v}\}
\end{eqnarray}

Intuitively, by inverting $\mbf A$, the small magnitude eigenvalues become the large ones
of $\mbf A^{-1}$.
The resulting $\mbf H'_{m}$ is likely to capture these
eigenvalues first. 
Based on Arnoldi algorithm, 
the inverted Krylov subspace has the relation 
%in pratical computation.
\begin{eqnarray}
 \mbf{A}^{-1}\mbf{V_m} =  
     \mbf V_m \mbf H'_m + 
     h'_{m+1,m} \mbf v_{m+1}\mbf e_m^\mathsf{T} 
\end{eqnarray}

The matrix exponential $e^{\mbf A} \mbf v$ is calculated as
%$\left | \beta \right| \mbf V_m \mbf e^{h\mbf H'^{-1}_m}\mbf e_1$.
\begin{eqnarray}
 e^{\mbf A} \mbf v\ \approx \lVert \mbf v \rVert \mbf V_m e^{h\mbf {H'}^{-1}_m} \mbf e_1 ,
\end{eqnarray}

To put this method into Alg. \ref{algo:arnoldi_std} just 
by using $\mbf C$ instead of $\mbf G$ the input variables. 
and LU decompose $ \mbf G$.
 %for the LU decomposition,
%$[\mbf L,\mbf U] =  \text{LU\_Decompose}(\mbf G)$, 
%and $\mbf X_2 = \mbf C$.  
In the line $15$ of Alg. \ref{algo:arnoldi_std}, $\mbf H_m = \mbf {H'}^{-1}_m$.
The posterior error approximation 
%$\lVert \mbf r_m(h) \rVert $ is  
\begin{eqnarray}
\label{eq:err_inverted_krylov}
  \lVert \mbf r_m(h) \rVert 
  =
  \lVert \mbf v  \rVert
  \left |  \mbf A  h'_{m+1,m} \mbf v_{m+1} 
  \mbf e^T_m {\mbf H'}^{-1}_{m}
  e^{h {\mbf H'}^{-1}_{m}}
  \mbf e_1 \right |
\end{eqnarray}
which is derived from the residual-based error approximation 
\cite{Botchev12}.
%When the $\mbf A$ has large condition number and densely distributed spectrum,
When the matrix $\mbf A$ has large condition number, the convergence rate 
might be slow to generate the inverted Krylov subspace basis. 
%In the next subsection, we solve this problem 
%by confining the specturm of
%using shift-and-invert Krylov subspace \cite{Van06, Moret04},

\subsection{Matrix Exponential Computation using Extended Krylov Subspace (E-MEXP)}

Chen \emph{et. al.} proposed to use Extended Krylov Subspace 
and try to place a 
balance between computational efficiency and accuracy,
which tries to avoid the relatively dense matrix $\mbf G$ compared to $\mbf C$.  

The idea is building Krylov subspace with standard $\mbf A$ and $\mbf A^{-1}$ at the
same time. The later one is constructed after every $k$ vectors with $\mbf A$. 
\begin{eqnarray}
K_{m,km} = \text{span}\{\mbf v, \mbf {Av}, \mbf {A}^2 \mbf v, \cdots, \mbf{A}^k \mbf v 
, \mbf{A^{-1}} \mbf{ v},
\\ \nonumber 
\mbf {A}^{k+1} \mbf {v},\cdots, \mbf {A^{2k}} \mbf{v},  \mbf{A}^{-2} \mbf{v},  \cdots,  % \mbf{A}^k \mbf v ,
\\ \nonumber 
\mbf{A}^{k(m-1)} \mbf v\cdots, \mbf{A}^{-m+1} \mbf v
\}
\end{eqnarray}
When $k = 0$, it is I-MEXP; when no $A^{-1}$ is needed, it backs to S-MEXP.

The recursive relation to obtain a new basis vector is given below,
\begin{eqnarray}
\text{if~} n=1 \text{~or~} mod(n,k+1) = 2, \cdots, k
\\ \nonumber
h_{n+2,n+1} \mbf v_{n+1} = \mbf A \mbf v_n - \mbf V_n h_{1:n,n}
\\ \nonumber
\text{if~}  mod(n,k+1) = 0
\\ \nonumber
h_{n+1,n} \mbf v_{n+1} = \mbf A \mbf v_n - \mbf V_n h_{1:n,n}
\end{eqnarray}
\begin{algorithm}
\label{algo:extended_krylov}
\caption{Arnoldi process in MEXP with Extended Krylov Subspace}
%$\rm K_m(\mbf X_1^{-1}\mbf X_2, \mbf v)$} %~\cite{Weng12_TCAD, Weng12_ICCAD}}
\KwIn{ $\mbf L, \mbf U, \mbf X_2, h ,\mbf x(t),  \epsilon $  }
%\KwOut{ $\mbf V_m, \mbf H_m,  m$ }
\KwOut{ $\mbf x(t+h)$ }
    {   
%	[$\mbf L, \mbf U$]=LU($\mbf X_1$)\\
%	Normalize the intial vector 
	$\mbf v = \mbf x(t), \mbf v_1 = \frac{\mbf v }{\lVert \mbf v \rVert}$\;
	\For  {$j=1:m$}
	{
	   % Calculate 
%	    $   \mbf w =  \mbf X_1^{-1} \mbf X_2 \mbf v_{j} $ by solving
	    $\mbf w = \mbf U^{-1}  (\mbf L^{-1} (\mbf X_2 \mbf v_{j})) $ \;
	    \For {$i = 1:j$}
	    {
	%	Orthogonalization 
		$h_{i,j} = \mbf w^T\mbf v_{j}$\;
		$\mbf w = \mbf w - h_{i,j} \mbf v_{j}$\;
	    }
	    $h_{j+1,j} = \lVert \mbf w \rVert $\;
	    $\mbf v_{j+1} = \frac{\mbf w }{h_{j+1,j}} $\;
	    % \If {$ h_{i+1,j} < \epsilon $}
	    \If {$ || \mbf r_j(h)|| < \epsilon $}
	    {
		$m = j$\;
		break\;
	    }
	}
	$\mbf x(t) = \lVert \mbf v \rVert \mbf {V_m} e^{h \mbf H_m} \mbf e_1 $\;
	%$\lVert r_m(h) \rVert  =  \lVert \mbf v \rVert \left| h_{m+1,m} e_m^T e^{h\mbf H_m} e_1 \right|$
    }
\end{algorithm}



==> sub-mexp_method.tex <==
MEXP\cite{Weng11_ASICON}\cite{Weng12_TCAD} is based on the analytical solution of~(\ref{eqn:ode}).
With initial solution 
%$\mbf{x}(0)$ 
from the DC analysis via direct\cite{Davis06} or iterative approaches\cite{Saad03}, the equation 
of MEXP from $t$ to $t+h$ can be expressed as
\begin{eqnarray} 
    \label{eqn:discrete_sol}
    \mbf{x}(t+h) = e^{\mbf{A}h}\mbf{x}(t) + \int^{h}_{0}e^{\mbf{A}(h-\tau)}\mbf{b}(t+\tau)d\tau.
\end{eqnarray}
where $\mbf{A} = - \mbf{C}^{-1}\mbf{G}$, and $\mbf{b}(t) = \mbf{C}^{-1}\mbf B\mbf{u}(t)$, when $\mbf{C}$ is not singular.
%Section~\ref{sec:rational_krylov} will show that the regularization process can be avoided. 
Assuming that input $\mbf{u}(t)$ is piece-wise linear (PWL), we integrate the last term in 
(\ref{eqn:discrete_sol}) analytically, turning the solution into the sum of three terms associated 
with matrix exponential operators,
\begin{eqnarray} 
\label{eqn:pwl_exact_sol}
    \mbf{x}(t+h)&=& e^{\mbf{A}h}\mbf{x}(t) \nonumber \\
		&+& (e^{\mbf{A}h} - \mbf{I})\mbf{A}^{-1}\mbf{b}(t) \nonumber \\
	        &+& (e^{\mbf{A}h}-(\mbf{A}h+\mbf{I}))\mbf{A}^{-2}\frac{\mbf{b}(t+h)-\mbf{b}(t)}{h}.
\end{eqnarray}
Eqn. (\ref{eqn:pwl_exact_sol}) has three matrix exponential terms, which are generally referred 
as $\varphi$-functions of the zero, first and second order~\cite{Niesen11}. It has been shown in 
\cite[Theorem 2.1]{Almohy11} that one can obtain the sum of them in one shot by computing the exponential 
of a slightly larger $(n+p)\times (n+p)$ matrix, where $n$ is the dimension of $\mbf{A}$, and $p$ is the 
order of the $\varphi$-functions ($p = 2$ in (\ref{eqn:pwl_exact_sol})). Thus, (\ref{eqn:pwl_exact_sol}) 
can be rewritten into
\begin{equation}
\label{eq:one_exp}
\mbf{x}(t + h) = \left[ 
			\begin{array}{*{20}{c}}
			    \mbf{I}_n & \mbf 0
			\end{array} 
		 \right]
		 e^{\mbf {\widetilde A} h}
		 \left[ 
			\begin{array}{*{20}{c}}
			    \mbf{x}(t)	\\
	    			\mbf    e_2
			\end{array} 
		\right],
\end{equation}
with
\begin{equation}
    \begin{gathered}
	\mbf {\widetilde A} = \left[ 
			 \begin{array}{*{20}{c}}
			    \mbf{A} & \mbf{W} \\
			    \mbf{0} & \mbf{J}
			\end{array} 
		   \right],\;\;\;
	\mbf{W} = \left[ 
			\begin{array}{*{20}{c}}
			    \frac{\mbf{b}\left(t + h \right) - \mbf{b}\left( t \right)}{h} & \mbf{b}\left( t \right)
			\end{array} 
		  \right] \hfill \\
	\mbf{J} = \left[ 
			\begin{array}{*{20}{c}}
			    0 & 1 \\
      			    0 & 0
			\end{array} 
		  \right],\;\;\;\;\;\;\;\;
\mbf e_2 = \left[ 
		    \begin{array}{*{20}{c}}
			0 \\
      			1
		    \end{array} 
	      \right] \hfill \\
    \end{gathered}
\end{equation}
To keep the notations simple, we use 
%$\mbf{A}$ and 
$\mbf{v}$ to represent 
% $\mbf{A}'$ and 
$[\mbf{x}(t)\;\; \mbf e_2]^\mathsf{T}$ in the rest of paper, respectively. 
Note that the kernel computation of MEXP is to derive the exponential of a matrix, i.e., $e^\mbf{A}\mbf{v}$, 
which is approximated by the Krylov subspace method in works~\cite{Weng12_TCAD}\cite{Weng11_ASICON}. 
The Krylov subspace method has better scalability mainly from its sparse matrix-vector product centric computation. 
However, such approximation is only better for those eigenvalues with small magnitude, which 
means the maximum step size of MEXP in a stiff circuit has to be constrained in order to maintain the accuracy of 
approximation. In the following section, we will present how the rational basis could relax the stiffness constraint.


\subsection{Advantages of ETD}

ETD is an A-stable method 
when eigenvalues of $\mbf A$ are negative~\cite{Weng12_TCAD}.
The step size $h$ of ETD is limited by the computation error of matrix 
exponential and PWL assumption.
In the perspective of approximation, it is theoritically different from 
%\emph{i.e.}, 
FE, BE, and TR methods. 
These methods approximate Eqn. (\ref{eqn:ode}) by 
polynomial expansions in Taylor series
and drop high-order terms.
%On the other hand, t
Therefore, the step size $h$ is restricted by LTE and stability.

On contrary, ETD solves the equations analytically.
Given a possible step region under PWL
when wider than the traditional methods,
ETD can enjoy larger time stepping. 
%than FE, BE and TR. 
It is because that analytical solution of Eqn. (\ref{eqn:ode})
and Eqn. (\ref{eqn:pwl_exact_sol}) contains the input sources information. 
When the step region is limited by multiple transitions of input sources, 
which violates the PWL,  
the simulation work can be divided into
serveral sub-taskes by seperating the input sources.
By doing this, 
given subset of input sources to the same circuit system, 
it helps recover suitable stepping region. % for MATEX doing time marching. 
Section VI proposes an efficient framework to handle sub-tasks 
%and solve individual, than
and parallel process them with the help of superposition property in linear systems.
Additionally, the adaptive time controlling is also very straightforward in
ETD, which is discussed in Section IV.


\subsection{Nonlinear Circuit Simulation Formulation}




==> sub-nonlinear.tex <==


Previous nonlinear circuit simulation using matrix exponential method \cite{Weng12_TCAD} is restricted by
the stiff component in the system, also requires regularization process for $\mbf C$ in order to 
remove the singularity for the matrix factorizations \cite{Chen12_TCAD}.


\subsection{Formulation}

For simplicity, first we formulate circuit simulation problem into  
\begin{eqnarray}
\frac{d\mbf x(t)}{dt}  = f(\mbf x(t),\mbf u(t))
\end{eqnarray}
where $\mbf x(t)$ is the voltage and current at time $t$. $\mbf u(t)$ is the input in time $t$. 
Traditionally, it uses BDF to solve the system. 

In matrix exponential method, exponential Rosenbrock-type methods \cite{Hochbruck10_EXP}\cite{Hochbruck09_RB} are often resorts to solve such nonlinear system,
%the first order Rosenbrock method is shown as follows,
For autonomous problem, 
a so-called exponential Rosenbrock-Euler method %\cite{Hochbruck10_EXP}\cite{Hochbruck09_RB} 
is given by 
\begin{eqnarray}
\label{eq_rbeuler}
\mbf x_{n+1} & = & e^{h_n \mbf J_n} \mbf x_n + h_n \phi_1(h_n\mbf J_n) g_n(\mbf x_n) \nonumber \\
 &=&\mbf x_n + h _n \phi_1(h_n\mbf A) F_n( \mbf x_n) 
\end{eqnarray} 
For non-autonomous problem, 
\begin{eqnarray}
\label{eq_rbna}
\mbf x_{n+1} %& = & e^{h_n \mbf A} \mbf x_n + h_n \phi_1(h_n\mbf A) g_n(\mbf x_n) \nonumber \\
 =\mbf x_n + h _n \phi_1(h_n\mbf J_n) F_n( \mbf x_n)
 + h_n^2\phi_2(h_n \mbf J_n) \mbf v_n  
\end{eqnarray}
where
\begin{eqnarray}
\mbf J_n = \frac{\partial f}{\partial \mbf x} (t_n, \mbf x_n), ~~
\mbf v_n = \frac{\partial f}{\partial \mbf x} (t_n, \mbf t),\nonumber \\   
\phi_1(h_n \mbf J_n) = \frac{e^{h_n \mbf J_n} - \mbf I}{h_n \mbf J_n}, ~~
\phi_2(h_n \mbf J_n) = \frac{ \phi_1(h_n \mbf J_n) - \mbf I}{h_n J_n}, \nonumber \\
\phi_3(h_n \mbf J_n) = \frac{ \phi_2(h_n \mbf J_n) - \frac{1}{2}\mbf I}{h_n J_n}
\end{eqnarray}


It is a second order exponential Roseenbrock-type method.
The advantage of Eq. \ref{eq_rbeuler} is that the stable in the entire complex plan, which is superior to all
of the BDF methods.
Therefore, the $\phi$ function permit a large value for the step size $h_n$ \cite{Carr13}.




\begin{algorithm}[h]
\label{algo:mexph}
\caption{Circuit simulation using Exponential Rosenbrock-Euler method (fixed step size)}
\KwIn{Circuit systems}
%\KwIn{ $ \mbf C, \mbf G , \mbf B, \mbf u(t), \tau, \gamma$  
%}
%\KwOut{ $\mbf V_m, \mbf H_m,  m$ }
\KwOut{  $\mbf x$ from $[0, T]$}
{   
%	[$\mbf L, \mbf U$]=LU($\mbf X_1$)\\
%	Normalize the intial vector 
	$t=0$\;
	%obtain DC solution\;
	%$s=T_{start}$\;
	$\mbf x(t) =$  DC\_analysis\;  
	\While{transient simulation}{
	Evaluate devices, obtain $\mbf C_{nl}, \mbf G_{nl}, I_{nl}$\;
	Obtain $\mbf J_n = \frac{\partial f}{\partial u} (t_n, \mbf x_n) = -(\mbf C_l + \mbf C_{nl})^{-1} (\mbf G_l + \mbf G_{nl})$\;
	Compute term $v_n$ with respect to input sources
	 $\mbf v_n = \frac{\partial f}{\partial t} (t_n, \mbf x_n) = -(\mbf C_l + \mbf C_{nl})^{-1}  \frac{d\mbf b(t_n)}{dt} $ \;
	 Compute $g_n(\mbf x_n) = (\mbf C_l + \mbf C_{nl})^{-1} I_{cur}$\;
 	 $\phi_1(h_n \mbf J_n) = \frac{e^{h_n J_n} - \mbf I}{h_n J_n}$\; 
	 $\phi_2(h_n \mbf J_n) = \frac{ \phi_1(h_n \mbf J_n) - \mbf I}{h_n J_n}$\;
	 $\phi_3(h_n \mbf J_n) = \frac{ \phi_2(h_n \mbf J_n) - \frac{1}{2}\mbf I}{h_n J_n}$\;
	 Compute 
	 $\mbf x_{n+1} =\mbf x_n + h _n \phi_1(h_n\mbf A) F_n( \mbf x_n)
	  + h_n^2\phi_2(h_n \mbf A) \mbf v_n $\;
$t=t+h_n$\;
}
}
\end{algorithm}


\subsection{Formulation for MNA-based Circuit Simulation}

$\mbf J_n$ is always with exponential term or inversion operation. 
Therefore, the Krylov subspace method is used toDAC approximate $\mbf J_n$ in order to 
avoid $\mbf C$ inversion. The benefit of this is that $\mbf C$ is likely to be singular matrix during the simulation. Furthermore, in some post-layout simulation, the $\mbf C$ is relative dense compared to non post-layout version as well as $\mbf G$.
\begin{eqnarray}
(\mbf C_l + \mbf C_{nl} ) 
\frac{d \mbf x(t)}{dt} + 
(\mbf G_l + \mbf G_{nl} ) \mbf x(t)  
= \mbf B \mbf u(t)  + \mbf I_{cur}
\end{eqnarray}
\begin{eqnarray}
\mbf C  
\frac{d \mbf x(t)}{dt} + \mbf G \mbf x(t)  
= \mbf B \mbf u(t)  + \mbf I_{cur}
\end{eqnarray}
\begin{eqnarray}
\frac{d \mbf x(t)}{dt} + \mbf C^{-1} \mbf G \mbf x(t)  
= \mbf C^{-1} \mbf B \mbf u(t)   + \mbf C^{-1} \mbf I_{cur}
\end{eqnarray}
\begin{eqnarray}
\frac{d \mbf x(t)}{dt} - \mbf J \mbf x(t)  
 =  \mbf b(t)  + \mbf g_n(\mbf x)
\end{eqnarray}
The components for the above systems 
\begin{eqnarray}
\mbf J_n = -\mbf C^{-1} \mbf G , ~~
\frac{1}{\mbf J_n}=-\mbf G^{-1} \mbf C
\end{eqnarray}
where $\mbf C = \mbf C_l + \mbf C_{nl}$, $\mbf C_{nl}$ is the capactiance matrix from nonlinear devices.
$\mbf G_{nl}$ is the conductance matrix from nonlinear devices.
\begin{eqnarray}
\mbf g_n(\mbf x_n) = \mbf C^{-1} \mbf I_{cur}(\mbf x_n) 
%, ~~\frac{1}{\mbf J_n}=-\mbf G^{-1} \mbf C
\end{eqnarray}
\begin{eqnarray}
\phi_1(h_n \mbf J_n) = - \frac{1}{h_n} (e^{h_n \mbf J_n} -\mbf I)\mbf G^{-1} \mbf C
\end{eqnarray}
\begin{eqnarray}
\phi_2(h_n \mbf J_n) = - \frac{1}{h_n} (\phi_1(h_n \mbf J_n) -\mbf I)\mbf G^{-1} \mbf C
\end{eqnarray}
\begin{eqnarray}
\phi_3(h_n \mbf J_n) = - \frac{1}{h_n} (\phi_2(h_n \mbf J_n) -\frac{1}{2}\mbf I)\mbf G^{-1} \mbf C
\end{eqnarray}
\begin{eqnarray}
F_n(h_n \mbf J_n) = \mbf J_n \mbf x_n + g_n(\mbf x_n) + \mbf b(t_n) 
\end{eqnarray}
 \begin{eqnarray}
 && \mbf x_{n+1}
 \nonumber \\
 \begin{comment}
  &=& \mbf x_n +(-1) (e^{h_n \mbf J_n} -\mbf I)\mbf G^{-1} 
 ( \mbf x_n +  \mbf I_{cur}(\mbf x_n) +  \mbf Bu(t_n) ) \nonumber \\
  &+& h_n^2\phi_2(h_n \mbf J_n) \mbf v_n  \nonumber \\
  &=& \mbf x_n +(-1) (e^{h_n \mbf J_n} -\mbf I)\mbf G^{-1} 
   ( \mbf x_n +  \mbf I_{cur}(\mbf x_n) +  \mbf Bu(t_n) ) \nonumber \\
    &+& (-1)h_n(\phi_1(h_n \mbf J_n) -\mbf I )\mbf G^{-1}\mbf B  \frac{ \mbf b(t+h_n) - \mbf b(t)}{h_n} \nonumber\\   
    \end{comment}
&=& \mbf x_n + (e^{h_n \mbf J_n} -\mbf I)(-\mbf G^{-1}) 
       (-\mbf G \mbf x_n +  \mbf I_{cur}(\mbf x_n) +  \mbf Bu(t_n) ) \nonumber \\
  	&+&  ( (e^{h_n\mbf J_n} -\mbf I)((\mbf G^{-1} \mbf C)
    - h_n  \mbf G^{-1} \mbf C )\mbf G^{-1} \mbf B  \frac{ \mbf u(t+h_n) - \mbf u(t)}{h_n} \nonumber  \\
&=& \mbf x_n + (e^{h_n \mbf J_n} -\mbf I) 
           (\mbf x_n -  \mbf G^{-1}( \mbf I_{cur}(\mbf x_n) +  \mbf Bu(t_n) ) ) \nonumber \\
   &+&  ( (e^{h_n\mbf J_n} -\mbf I) \mbf G^{-1} \mbf C\mbf G^{-1} \mbf B  \frac{ \mbf u(t+h_n) - \mbf u(t)}{h_n} \nonumber  \\
   &+ & h_n  \mbf G^{-1} \mbf C \mbf G^{-1} \mbf B  \frac{ \mbf u(t+h_n) - \mbf u(t)}{h_n}  
\end{eqnarray} 
 There are two matrix exponential and vector products to evaluate $e^{h_n \mbf J_n} \mbf v_1
 $ and $e^{h_n\mbf J_n}\mbf v_2$ where 
 \begin{eqnarray}
 \mbf v_1 =  \mbf x_n -  \mbf G^{-1}( \mbf I_{cur}(\mbf x_n) +  \mbf Bu(t_n) ) 
 \nonumber 
 \\
 \mbf v_2 = \mbf G^{-1}\mbf C  \mbf G^{-1}\mbf B  \frac{ \mbf u(t+h_n) - \mbf u(t)}{h_n}
 \end{eqnarray}
 The good thing about exponential Rosenbrock-Euler method is that  
 $\mbf J_n$ is maintained, only by changing step size $h_n$.
 It is 
 quite different from BDF methods, which 
 update the linear system with different time step size.  

\subsection{Krylov subspace methods for Nonlinear circuit simulation}

The standard Krylov subspace \cite{Weng12_TCAD} has a limitted scope of circuit, which is for mild system. 
In the practical application of circuit simulation, the elements in matrix, especially in $\mbf C$, quite differ. 
For example, device capacitance range and wire capacitance range sometimes varied in magnitudes.
Even dealing the simple linear circuit system \cite{Zhuang14_DAC}. 
Therefore, the matrix exponential method \cite{Weng12_ICCAD} \cite{Weng12_TCAD} using explicit $\mbf C$ inversion tend to converge very slow and consume huge memory.
In this paper, we focus on inverted Krylov and rational Krylov subspace. 

%The importance of the Krylov subspace here is due to the element value. 

\subsection{Error Estimations}
{\bf Krylov approximation error}
for adaptive stepping control ... 

{\bf Nonlinear error control}
When strong nonlinear happens ... 

\subsection{Circuit simulation using exponential Rosenbrock-Euler method and Krylov subspace with adaptive stepping}
The algorithm:
\begin{algorithm}[h]
\label{algo:mexph}
\caption{Circuit simulation using exponential Rosenbrock-Euler method and Krylov subspace with adaptive stepping}
\KwIn{Circuit systems}
%\KwIn{ $ \mbf C, \mbf G , \mbf B, \mbf u(t), \tau, \gamma$  
%}
%\KwOut{ $\mbf V_m, \mbf H_m,  m$ }
\KwOut{  $\mbf x$ from $[0, T]$}
{   
%	[$\mbf L, \mbf U$]=LU($\mbf X_1$)\\
%	Normalize the intial vector 
	$t=0$\;
	%obtain DC solution\;
	%$s=T_{start}$\;
	$\mbf x(t) =$  DC\_analysis\;  
	\While{transient simulation}{
	Evaluate devices, obtain $\mbf C_{nl}, \mbf G_{nl}, I_{nl}$\;
	Obtain $\mbf J_n = \frac{\partial f}{\partial u} (t_n, \mbf x_n) = -(\mbf C_l + \mbf C_{nl})^{-1} (\mbf G_l + \mbf G_{nl})$\;
	\While{1}{
	Compute term $v_n$ with respect to input sources
	 $\mbf v_n = \frac{\partial f}{\partial t} (t_n, \mbf x_n) = -(\mbf C_l + \mbf C_{nl})^{-1}  \frac{d\mbf b(t_n)}{dt} $ \;
	 Compute $g_n(\mbf x_n) = (\mbf C_l + \mbf C_{nl})^{-1} I_{cur}$\;
 	 Krylov subspace for $\phi_i$:
 	 $\phi_1(h_n \mbf J_n) $,
	 $\phi_2(h_n \mbf J_n) $,
	 $\phi_3(h_n \mbf J_n)$\;
	 Compute 
	 $\mbf x_{n+1} =\mbf x_n + h _n \phi_1(h_n\mbf A) F_n( \mbf x_n)
	  + h_n^2\phi_2(h_n \mbf A) \mbf v_n $\;
	 Compute error estimation\;
	 \If{error meets the criteria}{ 
	 $h_n = 2h_n$\;
	 break\;
	 }
	 \Else{
	 $h_n = h_n/2$\;
	 }	 
	 }
	 $t=t+h_n$\;
	}	
}
\end{algorithm}


==> sub-pwr_grid_formulation.tex <==
%DO WE NEED A POWER GRID FIGURE TO SHOW MORE DETAILS ABOUT THE FORMULATION?
\begin{comment}
Linear circuit can be formulated as a system of 
differential equations via modified nodal analysis as below:
\begin{eqnarray}
    \label{eqn:ode}
    \mbf{C}\dot{\mbf{x}}(t) = - \mbf{G}\mbf{x}(t) + \mbf{B}\mbf{u}(t),
\end{eqnarray}
where matrix $\mbf{C}$ describes the capacitance and inductance, matrix 
$\mbf{G}$ represents the resistance and the incidence between voltages 
and currents, and matrix $\mbf{B}$ indicates locations of the independent 
sources. Vector $\mbf{x}(t)$ describes the nodal voltages and branch currents 
at time $t$, and vector $\mbf{u}(t)$ represents the corresponding supply voltage 
and current sources associated to different blocks. 
%In order to stimulate the worst-case voltage noise, those current sources, which 
%represent the behavior of underlying blocks of a power grid, are often pre-characterized
%with pre-designed vectors. Many previous works\cite{Bodapati02}\cite{Du10}\cite{Ferzli10} 
%have developed different methodologies to generate worst-case stimulus currents.  
In this work, 
we assume those input sources are given and in the format of \emph{piece-wise linear}. 
\end{comment}

\subsection{Time Domain Formulation of Linear Cirsuits}
%\subsubsection{Formulation}
A linear circuit can be formulated as a system of 
differential algebraic equations (DAEs)
% Ordinary Differential Equations(ODEs) 
via modified nodal analysis (MNA),
\begin{eqnarray}
    \label{eqn:dae}
    \mbf{C}\dot{\mbf{x}}(t) = - \mbf{G}\mbf{x}(t) + \mbf{B}\mbf{u}(t),
\end{eqnarray}
where matrix $\mbf{C}$ describes the capacitance and inductance, matrix 
$\mbf{G}$ represents the resistance and the incidence between voltages 
and currents, and matrix $\mbf{B}$ indicates locations of the independent 
sources. $\mbf{x}(t)$ is a vector that describes the nodal 
voltages and branch currents 
at time $t$, and vector $\mbf{u}(t)$ represents 
the corresponding supply voltage 
and current sources associated to different blocks. 
%\subsection{Matrix Exponential Method}

To solve Eqn. (\ref{eqn:dae}) numerically,
it is, commonly, 
discretized with time step $h$ and transformed
to a linear algebraic system. 
%, respectively as follows: %based on different strategies as follows,
Then, given an initial condition $\mbf x(0)$ from DC analysis, 
or previous time step $\mbf x(t)$,
% of circuit and
%$h$ is the size of time step,
$\mbf x(t+h)$ can be obtained by traditional FE, BE, TR Method
and 
exponential time differencing with matrix exponential method 
 as follows.
%\subsection{Linear One-Step Methods}
\begin{itemize}
%\subsubsection{Forward Euler (FE) Method}
\item[(1)] 
{Forward Euler (FE) Method}
\begin{eqnarray}
    \label{eqn:fe}
     \frac{\mbf{C}}{h}  {\mbf{x}}(t+h) = (\frac{\mbf C}{h}- {\mbf G} ) \mbf{x}(t) + \mbf{B}\mbf{u}(t),
   % {\mbf{C}}  {\mbf{x}}(t+h) = ({\mbf C} - h{\mbf G} ) \mbf{x}(t) + h\mbf{B}\mbf{u}(t),
\end{eqnarray}
%where $h$ is the time-step in the discretization.
%\subsubsection{Backward Euler (BE) Method}
\item[(2)]
Backward Euler (BE) Method
\begin{eqnarray}
    \label{eqn:be}
   (\frac{\mbf{C}}{h} + {\mbf G}) {\mbf{x}}(t+h) = \frac{\mbf C}{h} \mbf{x}(t) + \mbf{B}\mbf{u}(t+h),
%    ({\mbf{C}} + h{\mbf G}) {\mbf{x}}(t+h) = {\mbf C} \mbf{x}(t) + h\mbf{B}\mbf{u}(t+h),
\end{eqnarray}
%\subsubsection{Trapezoidal (TR) Method}
\item[(3)]
Trapezoidal (TR) Method
\end{itemize}
\begin{eqnarray}
    \label{eqn:trap}
   (\frac{\mbf{C}}{h} + 
    \frac{\mbf G}{2}) {\mbf{x}}(t+h)  &&   \\ \nonumber
  =  (\frac{\mbf C}{h}-  \frac{\mbf G}{2} ) 
    \mbf{x}(t) & + & \mbf{B} \frac{ \left ( \mbf{u}(t) + \mbf{u}(t+h) \right)} {2}
  %  (2{\mbf{C}} + h{\mbf G}) {\mbf{x}}(t+h )  &   = & (2{\mbf C}- h{\mbf G} ) \mbf{x}(t) 
  %  \\ \nonumber
  % &+ & h\mbf{B}(\mbf{u}(t) +\mbf{u}(t+h))
\end{eqnarray}



==> sub-rational_krylov.tex <==

MEVP Krylov subspace approximation utilizes inverted basis \cite{Zhuang14_DAC} since standard Krylov subspace \cite{Weng12_TCAD} suffer two major problems. 
%a limitted scope of circuit, which 
%It is for mild system. 
In the practical application of circuit simulation, the elements in matrix, especially in $\mbf C$, quite differ. 
%For example, device capacitance range and wire capacitance range sometimes varied in magnitudes.
Even dealing the simple linear circuit system \cite{Zhuang14_DAC}. 
Therefore, the matrix exponential methods \cite{Weng12_ICCAD} \cite{Weng12_TCAD} using explicit $\mbf C$ inversion tend to converge very slow and consume huge memory.
In this paper, we focus on inverted Krylov and rational Krylov subspace. 
In this work, we utilize the Krylov basis with inverted basis,

\subsection{Inverted Krylov subspace methods for MEVP}
We construct the Krylov subspace as follows, 
\begin{eqnarray}
{\rm K_m}(\mbf A^{-1} , \mbf v) := \text{span}
{\{ \mbf v, \mbf A^{-1}\mbf v, \cdots, \mbf A^{-(m-1)} \mbf v}\}
\end{eqnarray} 
\begin{eqnarray}
\mbf A^{-1} \mbf V_m = \mbf V_m \mbf H_m 
+ \mbf H(m+1,m) \mbf v_{m+1} \mbf e_m
\end{eqnarray}
\begin{eqnarray}
 \mbf V_m^{T} \mbf A^{-1} \mbf V_m = \mbf H_m  
\end{eqnarray}
Then
\begin{eqnarray}
{\rm K_m}(-\mbf G^{-1}\mbf C , v) :=  \text{span} 
\{ \mbf v,  -\mbf G^{-1}\mbf C\mbf v,   \cdots,\nonumber \\  (-\mbf G^{-1}\mbf C)^{(m-1)} \mbf v \}
\end{eqnarray}
%The importance of the Krylov subspace here is due to the element value.
The solution to $\frac{d\mbf x}{dt} = \mbf A \mbf x$, $\mbf x_{n+1}(h) = e^{h\mbf A} \mbf x_n$.  
The matrix exponential and vector product 
\begin{eqnarray}
e^{h\mbf A}\mbf v =  e^{-h\mbf C^{-1}\mbf G}\mbf v \approx |\mbf v| \mbf V e^{h\mbf H_m^{-1}} \mbf e_1
\end{eqnarray}


\subsection{Error Estimation of Krylov Approximation For MEVP}

For Krylov subspace convergence and adaptive stepping controlling, the error estimation
is 
\begin{eqnarray}
\mbf x' = |\mbf v| \mbf V_m \mbf H_m^{-1} e^{h\mbf H} \mbf e_1   
\end{eqnarray}
The difference among the exact solution and approximated one is approximated as, which is derived from \cite{Botchev13},
\begin{eqnarray}
\mbf x' - \mbf x'_{exact} &=&  |\mbf v| \mbf V_m \mbf H_m^{-1} e^{h\mbf H} \mbf e_1 - \mbf A |\mbf v| \mbf V_m   e^{h\mbf H} \mbf e_1  \nonumber \\
&=&|\mbf v| (\mbf V_m \mbf H_m^{-1}  - \mbf A   \mbf V_m )  e^{h\mbf H} \mbf e_1  \nonumber \\
&=&|\mbf v| (\mbf A h_{m+1,m} \mbf v_{m+1})  e^{h\mbf H} \mbf e_1 
\end{eqnarray}
where $h_{m+1,m} = \mbf H(m+1,m)$.

The above error estimator contains $\mbf A$, which requires the inversion of $\mbf C$. However, we do not want this element due to singularity and extra inversion operations. 
In circuit simulator, the difference of derivates are not our primary concern.  $\mbf C x'- \mbf Cx_{exact}'$ is, which represents the phsycial meaning of node voltages and branch currents. By multiplication of $\mbf C$, we have 
\begin{eqnarray}
\mbf r_m(h) = \lVert  \mbf v \rVert |  h_{m+1,m} \mbf G \mbf V_{m+1} e^{h\mbf H_m^{-1}} \mbf e_1 |
\end{eqnarray}
The Arnoldi process is shown as {\bf{Algorithm \ref{algo_arnoldi}}}. 

\begin{algorithm}
\label{algo_arnoldi}
%\caption{Arnoldi process in Matrix Exponential-Based Circuit Simulation with Krylov subspace Method}
\caption{Arnoldi Algorithm with Inverted Krylov Subspace for Exponential Rosenbrock-Euler Circuit Solver}
%$\rm K_m(\mbf X_1^{-1}\mbf X_2, \mbf v)$} %~\cite{Weng12_TCAD, Weng12_ICCAD}}
\KwIn{ $\mbf A, \mbf x_n,  \epsilon, \mbf B,h, t$  }
%\KwOut{ $\mbf V_m, \mbf H_m,  m$ }
\KwOut{ $\mbf x_{n+1}, \mbf V_m, \mbf H_m, \mbf v, m$}
    {   
%	[$\mbf L, \mbf U$]=LU($\mbf X_1$)\\
%	Normalize the intial vector 
	%$\mbf v = \mbf x(t) + \mbf F(t,h) ,
	$\mbf v_1 = \frac{\mbf x_n }{\lVert \mbf x_n \rVert}$\;
	\For  {$j=1:m$}
	{
		Solve $\mbf A \mbf w = \mbf v_j$ \;
	    % Calculate 
		%	    $   \mbf w =  \mbf X_1^{-1} \mbf X_2 \mbf v_{j} $ by solving
	    %$\mbf w = \mbf U \backslash  (\mbf L \backslash (\mbf X_2 \mbf v_{j}))$
	    %{\tcc*[r]{a pair of forward and backward  substitutions}}
	    \For {$i = 1:j$}
	    {
	%	Orthogonalization 
		$h_{i,j} = \mbf w^T\mbf v_{i}$\;
		$\mbf w = \mbf w - h_{i,j} \mbf v_{i}$\;
	    }
	    $h_{j+1,j} = \lVert \mbf w \rVert $\;
	    $\mbf v_{j+1} = \frac{\mbf w }{h_{j+1,j}} $\;
	    % \If {$ h_{i+1,j} < \epsilon $}
	    \If {$ || \mbf r_j(h)|| < \epsilon $\label{alg1:conv1}} 
	    {
		$m = j$; break\; 
	    } 
	    %\label{alg1:conv2}
	}
%	$\mbf x(t+h) = \lVert \mbf v \rVert \mbf {V_m} e^{h \mbf H_m} \mbf e_1 $\;
	$\mbf x_{n+1} = \lVert \mbf v \rVert \mbf {V_m} e^{h \mbf H_m^{-1}} \mbf e_1$\;
	%$\lVert r_m(h) \rVert  =  \lVert \mbf v \rVert \left| h_{m+1,m} e_m^T e^{h\mbf H_m} e_1 \right|$
    }
%    \label{algo_arnoldi}
\end{algorithm}


\subsection{Nonlinear Error control}

When  nonlinear devices are taken intro considerations, the error estimation is derived, which is based on Eq. (3.2) of \cite{Caliari09_ER}, as follows,
\begin{eqnarray}
\label{eqn_nl_err}
  err  %\mbf {x_{n+1}} - \mbf x_{n+1}  \\
 &\approx&
h_n \phi_1 (h_n \mbf J_n) ( \mbf g(\mbf x_{n+1}) - \mbf g(\mbf x_n ) )  \\
&\approx  & - h_n \frac{e^{h_n \mbf J_n} -\mbf I}{h_n} \mbf G^{-1}\mbf C ( \mbf g (\mbf x_{n+1}) - \mbf g(\mbf x_n ) ) \nonumber \\
& \approx&  -\mbf V_m (e^{h_n \mbf H_n} -\mbf I) \mbf G^{-1}  ( \mbf I_{cur}(\mbf x_{n+1}) - \mbf I_{cur}(\mbf x_n ) )  \nonumber
\end{eqnarray}

When the $err$ is larger than error budget, the $h_n = \alpha h_n$, where $\alpha < 1$. Another good feature of our proposed method is there is no need to update the Krylov subspace, only by scaling the time step by the ratio $\alpha$ ($\alpha \le 1$). In the next section, we discuss the Krylov subspace for exponential Rosenbrock-Euler method, and its error estimations of Krylov subspace approximation of MEVP and nonlinear error control.
%\subsection{MEXER: Circuit Simulation using Exponential Rosenbrock-Euler Method and Krylov subspace with adaptive stepping}
The overall of algorithm is shown in {\bf{Algorithm. \ref{algo_erik}}}.

\begin{algorithm}[h]
\label{algo:mexph}
\caption{Proposed Nonlinear Circuit Solver}
\KwIn{Circuit systems (netlist)}
%\KwIn{ $ \mbf C, \mbf G , \mbf B, \mbf u(t), \tau, \gamma$  
%}
%\KwOut{ $\mbf V_m, \mbf H_m,  m$ }
\KwOut{Voltage and current solutions $\mbf x$ during time period $[0, T]$}
{   
%	[$\mbf L, \mbf U$]=LU($\mbf X_1$)\\
%	Normalize the intial vector 
	$t=0, n = 0$\;
	%obtain DC solution\;
	%$s=T_{start}$\;
	$\mbf x(t) =$  DC\_analysis\;  
	\While{transient simulation}{
	Evaluate devices based on $\mbf x(t)$, obtain $\mbf C, \mbf G , \mbf I_{nl}$\;
	Factorize $\mbf G$\;
	%Obtain $\mbf J_n = \frac{\partial f}{\partial u} (t_n, \mbf x_n) = -(\mbf C_l + \mbf C_{nl})^{-1} (\mbf G_l + \mbf G_{nl})$\;
    Compute term $\mbf v_1$ and use Krylov subspace approximations for $e^{h_n \mbf J_n}\mbf v_1$ of Eq. (\ref{eq_two_vec})\; 
     Compute $\mbf v_2$ and use Krylov subspace approximations for $e^{h_n \mbf J_n}\mbf v_2$ of Eq. (\ref{eq_two_vec})\; 
     $i = 0 $\;
     $\mbf x_i = \mbf x(t)$\;
	\While{true}{
	 Compute $\mbf x_{i+1}$ using Eq. (\ref{eq_solver})\;
	Evaluate devices based on $\mbf x_{i+1}$, obtain $\mbf I_{nl}(\mbf x_{i+1})$\;
	Compute error estimation by Eq. (\ref{eqn_nl_err})\;
	 \If{error meets the criteria}{ 
	 %Compute Eq. (\ref{eq_solver})\; 
	 $\mbf x(t+h) = \mbf x_{i}$\;
	 break\;
	 }
	 \Else{
	 $h = \alpha h$, such as $\alpha=1/2$\;
	 $i = i + 1$\;
	 }	 
	 }
	 $t=t+h$\;
	 	\If{iter $i$ small enough}{
	 		$h = 2h$\;
	 	}	
	}
}
\label{algo_erik}
\end{algorithm}

The exponential Rosenbrock-Type method is that  
 $\mbf J_n$ is maintained, only by changing step size $h_n$ to minimize the nonlinear error.
 It is 
 quite different from BDF methods, which 
 updates the linear system with different time step size, e.g. $(\mbf G+\mbf C/h)$.  
When the time step $h$ is changed from $h_n$ to $\alpha h_n$, we have 
\begin{eqnarray}
\label{solver_adpt}
\mbf x_{n+1}(\alpha h_n)& = &\mbf x_n - \mbf v_1 - \mbf v_2 %\nonumber \\
% &+& \alpha \mbf G^{-1} \mbf C \mbf G^{-1} \mbf B  ( \mbf u(t+h_n) - \mbf u(t) ) \nonumber \\
  + \alpha h_n \mbf v_2 \nonumber \\
 &+&  e^{\alpha h_n \mbf J_n}\mbf v_1 
 + e^{\alpha h_n \mbf J_n}\mbf v_2 
    \label{eq_solver_adpt}
\end{eqnarray}
 where  $x_{n+1}(\alpha h_n)$ is the solution at time $t_n+ \alpha h_n$. 


\subsection{Discussions}

Our proposed method is more robust SPICE-level general circuit simulation than our previous work \cite{Weng12_TCAD} %which mentioned in the Section IV. D, 
MEXP, which is suitable for moderately stiff problems due to the non-existent small valued capactitances. The time-consuming regularization process is totally removed even $\mbf C$ existed during the simulation.
It is due to the avoidance of factorize $\mbf C$. 

Besids that, this is advantageous  
in practice that the $\mbf C$ which results from circuit extraction \cite{Yu2013} 
may include many parasitic energe stroage elements with large variations in magnitude among them, which is often refered to strong coupling or post-layout/extraction simulation problems. This makes a denser $\mbf C$ compared to $\mbf G$. In our proposed method,
$\mbf J_n$ is always with exponential term or inversion operation. 
Therefore, the Krylov subspace method is used to approximate $\mbf J_n$ in order to 
avoid $\mbf C$ inversion. %The benefit of this is that $\mbf C$ is likely to be singular matrix during the simulation. Furthermore, in some post-layout simulation, the coupling effecst are extracted that make a denser $\mbf C$ compared to $\mbf G$. 
 
 And this is distinguished feature, that 
current SPICE-level simulators cannot afford, they always need to adapt
$(\beta \mbf C + \gamma \mbf G)$ in order to approximate transient behaviors of time domain circuits' response ($\mbf C/h+\mbf G$ in Backward Euler method, $\mbf C/h+\mbf G/2$ in Trapezoidal method, etc.).

The number of direct solving is reduced for time stepping. NRBE method requries at many LU solving during the iterations, while proposed method only needs one. The nonlinear error is controlled by the Eq. (\ref{eqn_nl_err}). This boosts the runtime performance since the LU decompsition is expensive when the circuit size is large in current IC designs. 





==> sub-results.tex <==

\begin{table*}[ht]
\begin{center}
\begin{tabular}{|l|l|l|l|l|l|l|l|l|l|}
	\hline
	\multicolumn{3}{|c|}{Designs} & \multicolumn{3}{|c|}{BENR} & \multicolumn{3}{|c|}{MATEX-ER} & \multirow{2}{*}{Speedup}
	\\ 
	\cline{1-9}
	PDN & \# Nodes  & \# Devices & \#Steps & \#LU  & Runtime(s)  & \#Steps  & \#LU  & Runtime(s) &  
	\\ \hline
	PDN & & & & & & & & &   \\ \hline	
	PDN & & & & & & & & &   \\ \hline
	PDN & & & & & & & & &    \\ \hline
PDN & & & & & & & & &   \\ \hline
PDN & & & & & & & & &   \\ \hline
PDN & & & & & & & & &   \\ \hline
\end{tabular}
\end{center}
\end{table*}

{\color{red}
The algorithms are implemented in MATLAB and C/C++, where all devices are evaluated using the BSIM3 model. The interacts between C/C++ and MATLAB via MEX. Our tests include modified IBM and Synopsys Inc.'s internal testcases's circuits.

%{\color{red} add ... e.g. what benchmarks to compare; what BDF; standard Krylov Matrix exponential. to test the large time step and post-layout handeling, buy time from dense $\mbf C$ factorization, but the convergent rate should be kept in mind.}

PDNs with gated transistors}



%\subsection{Power Distribution Networks with Gated Transistors} 


%\subsection{Test circuits: invertor chains ($s$-stage), ring Oscillators}


%\subsection{Post-layout-like circuits: dense capacitance matrices}


